Multi-Agent Safety Verification using Symmetry Transformations

We show that symmetry transformations and caching can enable scalable, and possibly unbounded, verification of multi-agent systems. Symmetry transformations map solutions and to other solutions. We show that this property can be used to transform cached reachsets to compute new reachsets, for hybrid and multi-agent models. We develop a notion of virtual system which define symmetry transformations for a broad class of agent models that visit waypoint sequences. Using this notion of virtual system, we present a prototype tool CacheReach that builds a cache of reachtubes for this system, in a way that is agnostic of the representation of the reachsets and the reachability analysis subroutine used. Our experimental evaluation of CacheReach shows up to 66% savings in safety verification computation time on multi-agent systems with 3-dimensional linear and 4-dimensional nonlinear fixed-wing aircraft models following sequences of waypoints. These savings and our theoretical results illustrate the potential benefits of using symmetry-based caching in the safety verification of multi-agent systems.

==> acknowledgment.tex <==
\section{Acknowledgments}
\label{sec:ack}
%\vspace{-.15in}
The authors are supported by a research grant from The Boeing Company and a research grant from NSF (CPS 1739966). We would like to thank John L. Olson and Arthur S. Younger from The Boeing Company for valuable technical discussions.
\vspace{-.2in}



==> exp_results.tex <==
\subsection{Setup and results}


==> hybridautomata.tex <==
\section{Hybrid Automata}
\label{sec:hybrid}


\section{Extension to agents with hybrid dynamics}

Different $f$s will represent different modes of operation of an agent. For example, taking-off, cruising, and landing modes of an aircraft or the different gears of a car. Formally, an agent would have a set $F = \{f_j: \mathbb{R}^n \times \mathbb{R}^m \times \mathbb{R}^+ \rightarrow \mathbb{R}^n\}$ of possible modes. This set would define the {\em type} of the agent.

- if there exists more than one agent type, we need a map from each agent type state to the "shared" space where safety would be defined.

- mention that our method can be extended to trajectory tracking controllers where instead of a mode we have an input signal.


\subsection{Agent hybrid dynamics}

A convenient way to model cyber-physical systems is using hybrid automata. A hybrid automaton models multiple modes of continuous dynamics that the agent switch between based on some conditions on its state and time~\cite{C2E2paper}.

%In this paper we consider a simplified version of hybrid automata with deterministic transitions, directed acyclic graph that models transitions between modes, and dynamics of all modes being modeled as (\ref{sys:input}).

For example, it can model the drone in Section~\ref{sec:single_drone_example} following a sequence of waypoints.
An {\em action} $a$ would change the parameter, and thus the mode of operation, of the dynamics.
% Each waypoint would be a separate mode where the mode is determined by the coordinates of the waypoint. 
 A condition under which an action $a$ is taken is called $Guard_a$. 
 The parameter may change once the action is taken. The change is defined a map called $\mathit{Reset}_a$.

In the drone waypoint following example, the action $a$ that would switch the drone from following the current waypoint $\mathit{wp}_o$ to following the next waypoint $\mathit{wp}_n$ would have: $Gaurd_a$ that is the predicate $(x,y) \in B(\mathit{wp}, \delta)$ that checks if the position of the drone is within a square around the waypoint and $\mathit{Reset}_a$ that is a map that sets $p$ in (\ref{sys:input}) to $\mathit{wp}_n$.

%Each mode is identified by a value of the parameter $p$ in (\ref{sys:input}).
We borrow the formal definition of a hybrid automaton from \cite{C2E2paper} while adapting it to our notations. Moreover, we remove the finiteness assumption on the number of modes and actions.

\sayan{Do we need actions $A$ or just unlabeled transitions are enough? This definition is much more general as it allws revisiting of ``waypoints'' or general transition graphs---not just sequences. Do we want that? Do we use that? If not there may be a simpler model. $f$ should be just a function of a certain type. Its {\em interpretation\/} is that it is the RHS of an ODE. This definition should be purely syntactic. Then, we define the semantics of the object. Executions, etc. It may make sense to have $guards: P \times P \rightarrow ?$ as an element of this object rather than the more general $D$}

\begin{definition}[modified version of Definition 1 in \cite{C2E2paper}]
\label{def:hybridautomata}
A Hybrid Automata $(HA)$ $\mathcal{A}$ is a tuple $\langle S, P, A, \disctrans, f \rangle$, where
\begin{enumerate}[label=(\alph*)]
%\item $V = X \cup \{loc\}$ is a set of variables. Here $loc$ is a discrete variable of finite type $Loc$. Valuations of $loc$ are called {\em locations}. Each $x \in X$ is a continuous variable of type $\mathbb{R}$. Elements of $val(V)$ are called states.
\item $S$ is the state $x$ space of continuous dynamics and $P$ is the parameter $p$ space that define the modes.
\item $A$ is a set of actions or transition labels.
\item $\disctrans \subseteq P \times A \times P$ is the set of discrete transitions. A transition $(p,a,p') \in \disctrans$ is written as $p \xrightarrow[]{a} p'$. The discrete transitions are described by finitely many guards and reset maps involving $p$.
\item $f$ is the right-hand-side of the differential equation~(\ref{sys:input}). It defines how the state evolves continuously with time for any given mode $p \in P$.
%\item $\trajs$ is a set of trajectories for $x$ which is closed under suffix, prefix and concatenation (see \cite{HuangM:HSCC2014} for details). For each $p \in P$, a set of trajectories $\trajs_p$ for parameter $p$ are specified by differential equation (\ref{sys:input}) and an invariant $I_l \subseteq val(X)$. Over any trajectory $\tau \in \trajs_l$, $\loc$ remains constant and the variables in $X$ evolve according to $E_l$ such that for all $t$ in the domain of $\tau$, $\tau(t)$ satisfies the invariant $I_l$.
\end{enumerate}
\end{definition}

Now that we defined the automata, we define what an execution would look like.

\begin{definition}[modified from \cite{C2E2paper}]
\label{def:ha_exec}
An execution of a hybrid automata $\mathcal{A}$ is an alternating sequence of trajectories and actions $\sigma = \xi_0 a_1 \xi_1 \dots $, where each trajectory $\xi_i$ is a solution of (\ref{sys:input}) and $\xi_i(x_i, p_i, t)=\xi_{i+1}(x_{i+1}, p_{i+1}, 0)$ and $t = \dur(\xi_i)$ is the last time point in $\xi_i$ before the switch. The duration of an execution is $\dur(\sigma) = \sum_{i}\dur(\xi_i)$. The number of switches in $\sigma$ in the time interval $[t_1,t_2]$ is $sw(\sigma, [t_1,t_2])$. The set of all executions that start from an initial set $\Theta$ and mode $p_0 \in P$ is denoted by $\mathit{execs}(\Theta, p_0)$. If we bound the maximum duration of the executions to be $T$ and the number of transitions between modes to be $J$, we denote the set by $\exec(\Theta, p_0,  T, J)$.
\end{definition}

Note from Definition~\ref{def:ha_exec} that a trajectory may satisfy a guard and still do not switch. Now we can define safety of the hybrid automaton with respect to an unsafe set.

\begin{definition}[Bounded time safety, \cite{C2E2paper}]
Given a hybrid automata $\mathcal{A}$ with an initial set $\Theta \subseteq S$, initial mode $p_0 \in P$, unsafe set $U$, time bound $T$, and number of transitions bound $J$, it is said to be unsafe, if there exists an execution $\xi_0 a_1 \dots \xi_k \in \exec(p_0, \Theta, T, J)$ such that $\xi_k(x_k,p_k, t) \in U$, where $t$ is the last time point in $\xi_k$. Otherwise, $\mathcal{A}$ is said to be safe. 
\end{definition}

We can define safety as well using reachsets and reachtubes. We define them first for $\mathcal{A}$.

\begin{definition}[Reachsets and reachtubes]
Given an initial set $\Theta \subset S$ and initial mode $p_0 \in P$, we define the reachset of hybrid automaton $\mathcal{A}$ over the time interval $[t_1,t_2]$ with maximum of $J$ switches as follows:
\begin{align}
	\reachset_{\mathcal{A}}(\Theta, p_0, J, [t_1,t_2]) = \{ x\ |\ \exists\ \sigma \in \mathit{execs}(\Theta,p_0), \sigma(t) = x, t \in [t_1, t_2], sw(\sigma, [t_1,t_2]) \leq J \}.
\end{align}
The unbounded time reachset is denoted by $\Reach(\Theta, p_0)$. When the reachable state is annotated with time, the result is a reachtube: $\Rtube_{\mathcal{A}}(\Theta, p_0, J, [t_1, t_2]) =  \{ (X,t) \ |\ X = \Reach_{\mathcal{A}}(\Theta, p_0, J, [t,t])\}$. The unbounded time reachtube is denoted by $\Rtube_{\mathcal{A}}(\Theta, p_0)$. An over-approximate reachset is a set $\AReach_{\mathcal{A}}(\Theta, p_0, J, [t_1, t_2]) \supseteq \Reach_{\mathcal{A}}(\Theta, p_0, J, [t_1, t_2])$ and an over-approximate reachtube $\ARtube_{\mathcal{A}}(\Theta, p_0, J, [t_1, t_2]) = \{(X_i, s_i)\}_{i=1}^{j}$, where $X_0 = \AReach_{\mathcal{A}}(\Theta, p_0, 0, [s_0, s_0])$, $X_i = \AReach_{\mathcal{A}}(\Theta, p_0,J_i, [s_{i-1},s_{i}])$, $\sum_{i=1}^{j} J_i \leq J$, and $s_0 = t_1 < s_1 < \dots < s_j = t_2$.
\end{definition}

Bounded time safety becomes a question if the intersection of the reachset or reachtube with the unsafe set is empty or not.
\begin{comment}
\begin{lemma}
	$\ARtube_{\mathcal{A}}(\Theta,p_0,[t_1, t_2])$ can be over-approximated by unioning  
	
	\hussein{Relate over-approximation of reachtubes of individual modes with the over-approximation of the tube of the automata. This will be essential to say that being able to compute a tube for individual modes is what matters for verification of hybrid automata.
	The rest of the lemma is just scratch that I'll modify.}
\begin{align}
\reachset_{\mathcal{A}}(\Theta, p_0, [t_1,t_2]) = \mathit{concat} (\langle \reachset(K_i,p_i,[t_i^b,t_i^e]) \rangle_{i=j_1}^{j_2}),
\end{align}
\begin{align}
	content...
\end{align}
where $K_{j_1} = \Reach_{\mathcal{A}}(\Theta,p_0,[t_1, t_1])$, $t_{j_1}^b = t_1 - \sum_{j=0}^{}$

\end{lemma}
\end{comment}

 
 
 \subsection{Example: Drone following a sequence of waypoints}
 \label{sec:agentplan}
 
 We design an automaton that models the drone in Section~\ref{sec:single_drone_example} following a sequence of waypoints. We start by defining the elements of the tuple in Definition~\ref{def:hybridautomata}. The state space $S$ is $\mathbb{R}^4$ since the state is
 %\{[10,3.2], [11.5, 7], [15, 8.5]$, $[18.5, 7.5] \}
  $(v,\psi,x,y)$, the parameter space is $P = \mathbb{R}^2$ since it represents the coordinates of waypoints in the plane, the action set is $A = \{ a_0, a_1, a_2  \}$, $D = \{ ([10,3.2], a_0, [11.5, 7])$, $([11.5, 7], a_1, [15, 8.5]), ([15, 8.5], a_2,[18.5, 7.5])\}$ and $f$ is the ODE shown in Section~\ref{sec:single_drone_example}. For any $a \in A$, the guard checks if the position of the drone is in the square of side equal to 0.5 around the waypoint that it transition from. For example, $Gaurd_{a_0} = (x, y) \in [[9.5,2.7],[10.5,3.7]]$. Moreover, for any $a \in A$, $\mathit{Reset}_{a}$ would set the value of the parameter $p$ to the following waypoint. For example, $\mathit{Reset}_a : p := [11.5,7]$.
 
 An initial set would be $\Theta = [[1,\frac{\pi}{4}, 5,-2], [2,\frac{\pi}{3}, 6,-1]]$. Now, consider a building that occupies the square $B = [[11.9,5.1],[12.9, 6.1]]$ in the plane.  An unsafe set would be the position of the drone be overlapping with the position of the building, i.e. $U = \{(v,\psi, x,y)\ |\ (x,y) \in B, v, \psi \in \mathbb{R}\}$.
 
%We  present an example of an agent tracking a sequence of goals.


%\sayan{This is not an example. What you mean to say that this is a special type of agent model that we will focus on this paper. Introduce it as such. Then give a real concrete example with ODEs and all.}
% For example, the waypoints an aircraft should reach sequentially to reach its destination or the sequence of segments of waypoints that the aircraft should fly over or parallel to. The set of possible goals is denoted by $W$ (for abstracted waypoints).
% \sayan{This is just a set, not a sequence? There is no additional structure?}
%  Each goal would be mapped to an input signal by the agent open loop controller $C : W \rightarrow (u: \mathbb{R}^{\geq 0} \rightarrow \mathbb{R}^m)$. It could be just a constant signal representing the goal.
 
% An agent would transition between goals based on conditions (guards) on its state and time that defines achievement of a goal $g$. 
% \sayan{Not clear what yo mean by transition. Can you go back and forth between goals? Type of $g$ is also not clear. Is it a subset of $R^n$ ? Discussion of SMT and first order logic is out of place here. We need a precise {\bf Definition} of this new type of agent model here.}
% These guards on transitions can be represented in first order logic and checked using a Satisfiability Modulo Theory (SMT) solver. The set of such guards is denoted by $G$. The sequence of pairs of a goal and corresponding condition on transitions of an agent is called a {\em plan} and denoted by $P$, where $P[i] = (w, g)$, $i \in \mathbb{N}$, $w \in W$ and $g \in G$.
 
% The input signal would be $C[P[i].w]$ till the guard $P[i].g$ is achieved. After which the agent switches to the following goal. Formally, $u(t) = C[P[0].w](t)$ for $t \in [0, t_1]$, where $t_1$ is the least time at which $x_1 = \xi(x_0, u, t)$ satisfy $P[0].g$. Generally, $u(t) = C[P[i].w](t - t_i)$ for $t \in [t_i, t_{i+1}]$, where $t_{i+1}$ is the time at which $\xi(x_i, u(t - t_i), t - t_i)$ satisfies $P[i].g$. Hence, $\xi(x_0, u, t) = \xi(x_i, u_i, t - t_i)$ for $t \in [t_i, t_{i+1}]$, where $t_i$ is the time at which the $(i-1)^{\mathit{th}}$ goal was achieved and $x_i = \xi(x_0, u, t_i)$.
 
 

 %\subsection{Unsafe set example: static obstacles}
 %A typical unsafe set $R$ for a system representing robot dynamics would be colliding with a static obstacle. For example, a drone colliding with a building. We can detect such collision by checking if the location of the agent is in, or in close proximity, to the building location. Given a set of coordinates $L \subseteq [N]$ in the state vector of an agent representing its physical location, the unsafe set would be $R \subseteq \mathbb{R}^{|L|}$ representing the physical occupancy of the building in the physical space.
 
% Hence, the input signal would be the concatenation of the input signals that guide the system to each of its goals. Formally, $u(t) = u_i(t - t_{i})$, where $i \in \mathbb{N}$, $u_i = C[P[i].w]$ and $t_{i}$ is the time at which the guard on the last transition $P[i-1].g$ was first satisfied.
 
 

%Thus, for a given plan $P$, we define the trajectory of the agent recursively:
%$\xi(x_0, u, t) = \xi(x_0, u_0, t)$ for $t \in [0, t_1]$, where $t_1$ 
% $\xi(x_0, u, t) = \xi(x_i, u_i, t - t_{i-1})$, where $x_i$ is the first time $\xi(x_0, u, \cdot)$ satisfies $i$ is the index of the current goal in the plan, $x_i$

%Hence, an agent dynamics would be defined by a tuple $A = \langle K, f, C, P \rangle$, where $G$ and $W$ are suppressed because the information needed is contained in $P$.

 
\subsection{Multi-agent dynamics}
\label{sec:multiagentdynamics}
%  $F_i = \{f_{i}^j: X_{i} \times U_i \times \mathbb{R}^{\geq 0} \rightarrow X_i \}_{j = 1}^{N_i}$
In this section, we will consider the case where multiple agents with the same mode dynamics exist in the same environment. Each of the agents is modeled using a hybrid automaton with different action set $A$, set of discrete transitions $D$, and initial set $\Theta$ but with the same state space $S$, parameter space $P$, and mode dynamics $f$.
For example, multiple drones of Example~\ref{sec:agentplan} may exist in a shared airspace following different sequences of waypoints to follow.

% They may be communicating with each other, and thus affecting each others' states.

Formally, we consider a system with $N$ agents. The $i^{\mathit{th}}$ agent dynamics is modeled using the hybrid automaton $\mathcal{A}_i$. We assume that for all $i \in [N]$, $\mathcal{A}_i.S = S$, $\mathcal{A}_i.P = P$, and $\mathcal{A}_i.f = f$. The rest of the components of the tuple along with the sets of initial states can be different between agents.

The resulting system can be modeled as a hybrid automaton $\mathcal{A}_c$ that results from the composition of $\{\mathcal{A}_i\}_{i=1}^N$, the hybrid automata of the agents. Then, $\mathcal{A}_c = \langle S_c, P_c, A_c, D_c, f_c \rangle$, where
\begin{enumerate}[label=(\alph*)]
\item $S_c = S \times S \dots \times S = S^N$ and $P_c = P^N$,
\item Let $a_c = (a_1, \dots a_N)$. Then, $a_c \in A_c$ iff for all $i\in [N]$, $a_i \in A_i$ or $a_i = \bot$, and $\exists j \in [N]$, $a_j \neq \bot$, 
\item Let $p_c = (p_1,\dots,p_N)$. Then, $(p_c,a_c,p_c') \in D_c$ iff $a_c[i] \neq \bot \implies (p_i,a_i,p_i') \in D_i$ and $a_c[i] = \bot \implies p_i = p_i'$, and 
\item $f_c = (f,\dots f) = f^N$, of length $N$.
\end{enumerate}
Moreover, guards would be the same for actions of individual agents. Formally, $Guard_{a_c} = \wedge_i Guard_{a_i}$ for all $i \in [N]$ such that $a_i \neq \bot$. A trajectory of $\mathcal{A}_c$ would be of the form $\xi_c(x_0, p, \cdot) = \prod_{i=1}^{N} \xi(x_{0,i},p_i,\cdot)$, where $x_{0,i}$ and $p_i$ are the initial state and parameter of the $i^{\mathit{th}}$ agent.

Moreover, given initial sets $\Theta_i \subseteq S$ and initial parameters $p_{i,0} \in P$, for $i \in [N]$, the initial set of $\mathcal{A}_c$ would be $\Theta_c = \prod_{i=1}^{N} \Theta_i$ and $p_{0,c} = ( p_{0,1}, p_{0,2}, \dots, p_{0,N})$.

Consequently,
\begin{align}
\AReach_{\mathcal{A}_c}(\Theta_c, p_0, J, [t_1, t_2]) &= \prod_{i=1}^{N} \Reach_{\mathcal{A}_i}(\Theta_i, p_{0,i}, J, [t_1, t_2]) \text{ and}\\ 
\ARtube_{\mathcal{A}_c}(\Theta_c, p_0, J, [t_1, t_2]) &= \prod_{i=1}^{N} \Rtube_{\mathcal{A}_i}(\Theta_i, p_{0,i}, J, [t_1, t_2]).
\end{align}  
Notice that we used $\AReach$ and $\ARtube$ since we are allowing each agent to have $J$ switches which can result in $NJ$ switches in $A_c$ which is larger than the allowed $J$ switches. We define approximate unbounded time reachset and reachtubes in a similar manner.

\begin{comment}

 % Each follows the same dynamics shown in (\ref{sys:input}).
  Given a compact initial set of states for each of the agents $K = \prod_{i=1}^N K_i \subset \mathbb{R}^{N \times n}$, we have the following system:
\begin{align}
\label{sys:multi}
\dot{X} = F(X,U(t), t),
\end{align}
where $X_0 \in K$, $U: \mathbb{R}^{\geq 0} \rightarrow \mathbb{R}^{N \times m}$, $F = (f, f, \dots f)$, and $f$ is that of system~(\ref{sys:input}). Its solution starting from $X_0 \in K$ is denoted by $\xi(X_0, U, \cdot)$.

Similar to Section~\ref{sec:agentplan}, the vector of input signals can be computed by a planner that assign each agent a plan to follow and a set of $N$ open loop controllers that create the corresponding input signals for the agents.

The reachset of the system would be the composed reachset of the individual agents. Formally, given a set of possible input signals $\mathcal{U} = \{ U : \mathbb{R}^{\geq 0} \rightarrow \mathbb{R}^{N \times m} \}$, 
\[\Reach(K, \mathcal{U},[t_1, t_2]) = \prod_{i=1}^{N} \Reach(K[i], \mathcal{U}[i],[t_1, t_2]).
\]
\end{comment}


\subsection{Example: Multiple drones following multiple sequences of waypoints}
In addition to the hybrid automata that models the dynamics of a drone following a predefined sequence of waypoints in Section~\ref{sec:agentplan}, we define another one that only differs in the sequence of waypoints that it follows. It has also a different initial set. Its set of actions is denoted by $A_2 = \{b_0, b_1 \}$ and the set of discrete transitions $D_2 = \{ ([13.3,5], b_0, [14, 8])$, $([14, 8], b_1, [17.2, 10])\} $. The guard of each action checks if the position of the drone $(x,y)$ in the plane is within a square of side 0.25 around next waypoint. Its initial set is $\Theta_2 = [[1,\frac{\pi}{4},2,0], [2,\frac{\pi}{3}, 3,1]]$.

Composing the two hybrid automata of the two drones result in $\mathcal{A}_c$. An unsafe set would be either of the drones positions crashing into the building in Section~\ref{sec:agentplan}. Another unsafe state would be the two drones crashing into each other. Hence, fix some $L_2$ distance $\epsilon > 0$ between the two drones below which the situation would be unsafe. Then, the unsafe set would be $U_c = \{ (v_1, \psi_1, x_1,y_1, v_2, \psi_2, x_2, y_2)\ |\ (x_1, y_1) \in B \text{ or } (x_2, y_2) \in B \text{ or } \| (x_1,y_1) - (x_2,y_2)\| \leq \epsilon$, $v_1,\psi_1, v_2, \psi_2 \in \mathbb{R}\}$.


%\subsection{Unsafe set example: dynamic obstacles}
%A typical unsafe set $R$ for such multi-agent system would be colliding agents. We can detect such collision by checking if the locations of the two agents are equal or in close proximity in the physical world at the same time. Given a set of coordinates $L \subseteq [N]$ in the state vector of an agent representing its physical location, 
%$R = \{(X,t)\ |\ X[i][L] = X[j][L], i,j \in [N], X = \xi(X_0, U, t), X_0 \in K, U \in \mathcal{U}, t \in [0,T] \}$.
% The projection of the state, input and dynamics vectors to the $i^{\mathit{th}}$ agent is denoted by $\pi_i(\cdot)$, i.e. $x_i = \pi_i(X)$, $$


% In addition to a plan for each agent, we have a connection graph that stores which agent's state affect which agent's state. The controller of an agent would map its plan and the states of the agents that are connected to it to an input signal of dimension $m$. 

% We consider a system with $N$ agent types. Each type $i \in [N]$, has a state space $X_i \subseteq \mathbb{R}^{n_i}$, an input space $U_i \subseteq \mathbb{R}^{m_i}$, and a set of $N_i$ possible modes of operation: $F_i = \{f_{i}^j: X_{i} \times U_i \times \mathbb{R}^{\geq 0} \rightarrow X_i \}_{j = 1}^{N_i}$. There are $A_i$ agents of each type. Each of the agents has a sequence  
% For each of the agents, we have two transformation functions $\gamma_i$ and $\rho_i$ such that:



==> inf_initset.tex <==
\subsection{Reachtubes starting from Infinite Initial Sets}
\label{sec:inf_initset}


==> prelude.tex <==
% !TEX root = main.tex
% marking changes

%\newcommand{\mitras}[1]{\textcolor{blue}{#1}}
\newcommand{\mitras}[1]{{#1}}
% for nomencl to produce page links
%\renewcommand*{\pagedeclaration}[1]{\unskip, \hyperpage{#1}}
%\renewcommand{\nomname}{List of Symbols and Functions}

\newcommand{\authcomment}[1]{\textbf{[[#1]]}}
\newcommand{\sayan}[1]{\textcolor{blue}{#1}}


%FIXED SETS

%\newcommand{\Time}{{\sf T}}                     %time domain
\newcommand{\nnt}{{\sf T}^{\geq 0}}             %nonnegative time points
\newcommand{\post}{{\sf T}^{>0}}                %positive time points
\newcommand{\Variables}{{\sf V}}                %variables

\newcommand{\num}[1]{\relax\ifmmode \mathbb #1\else $\mathbb #1$\fi}
\newcommand{\nnnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{\geq 0} \else ${\mathbb #1}_{\geq 0}$
  \fi}
\newcommand{\npnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{\leq 0} \else ${\mathbb #1}_{\leq 0}$
  \fi}
\newcommand{\pnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{> 0} \else ${\mathbb #1}_{> 0}$
  \fi}
\newcommand{\nnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{< 0} \else ${\mathbb #1}_{< 0}$
  \fi}
\newcommand{\plnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{+} \else ${\mathbb #1}_{+}$
  \fi}
\newcommand{\nenum}[1]{\relax\ifmmode 
  {\mathbb #1}_{-} \else ${\mathbb #1}_{-}$
  \fi}

\newcommand{\bools}{{\num B}}                    %reals
\newcommand{\reals}{{\num R}}                    %reals
\newcommand{\nnreals}{{\nnnum R}}                    %nonnegative reals
\newcommand{\realsinfty}{{\num R} \cup \{\infty, -\infty\}}                    %nonnegative reals
\newcommand{\plreals}{{\plnum R}}                    %positive reals
\newcommand{\naturals}{{\num N}}                      %natural numbers
\newcommand{\integers}{{\num Z}}                      %integers
\newcommand{\nnintegers}{{\nnnum Z}}    
\newcommand{\rationals}{{\num Q}}                      %rationals
\newcommand{\nnrationals}{{\nnnum Q}}                   % nonnegative rationals
\newcommand{\Time}{{\num T}}  


\newcommand{\R}{\mathbb{R}}

% ************** Sayan's New definitions will be added in this block START
% EXECUTIONS TRACES and FRAGS
\newcommand{\extb}[1]{\relax\ifmmode {\sf ExtBeh}_{#1} \else ${\sf ExtBeh}_{#1}$\fi} 
\newcommand{\tdists}[1]{\relax\ifmmode {\sf Tdists}_{#1} \else ${\sf Tdists}_{#1}$\fi} 

\newcommand{\exec}[1]{\relax\ifmmode {\sf Execs}_{#1} \else ${\sf Execs}_{#1}$\fi} 
\newcommand{\execf}[1]{\relax\ifmmode {\sf Execs}^*_{#1} \else ${\sf Execs}^*_{#1}$\fi} 
\newcommand{\execi}[1]{\relax\ifmmode {\sf Execs}^\omega_{#1} \else ${\sf Execs}^\omega_{#1}$\fi} 

\newcommand{\fintrace}[1]{\relax\ifmmode {\sf FinTraces}_{#1} \else ${\sf FinTraces}_{#1}$\fi} 

\newcommand{\trace}[1]{\relax\ifmmode {\sf Traces}_{#1} \else ${\sf Traces}_{#1}$\fi} 
\newcommand{\tracef}[1]{\relax\ifmmode {\sf Traces}^*_{#1} \else ${\sf Traces}^*_{#1}$\fi} 
\newcommand{\tracei}[1]{\relax\ifmmode {\sf Traces}^\omega_{#1} \else ${\sf Traces}^\omega_{#1}$\fi} 

\newcommand{\frag}[1]{\relax\ifmmode {\sf Frags}_{#1} \else ${\sf Frags}_{#1}$\fi} 
\newcommand{\fragf}[1]{\relax\ifmmode {\sf Frags}^*_{#1} \else ${\sf Frags}^*_{#1}$\fi} 
\newcommand{\fragi}[1]{\relax\ifmmode {\sf Frags}^\omega_{#1} \else ${\sf Frags}^\omega_{#1}$\fi} 

\newcommand{\reach}[1]{\relax\ifmmode {\sf Reach}_{#1} \else ${\sf Reach}_{#1}$\fi} 


\newcommand{\ball}[1]{\relax\ifmmode {\mathit{B}}_{#1} \else ${\mathit{B}}_{#1}$\fi} 

\newcommand{\untimexec}[1]{\relax\ifmmode {\sf Untimexecs}_{#1} \else ${\sf Untimexecs}_{#1}$\fi} 

\newcommand{\untimexecs}{{\untimexec{}}}
\newcommand{\execs}{{\exec{}}}
\newcommand{\traces}{{\trace{}}}
\newcommand{\fragss}{{\frag{}}}

\newcommand{\fexecs}{{\execf{}}}
\newcommand{\ftraces}{{\tracef{}}}
\newcommand{\ffragss}{{\fragf{}}}

\newcommand{\iexecs}{{\execi{}}}
\newcommand{\itraces}{{\tracei{}}}
\newcommand{\ifragss}{{\fragi{}}}
\newcommand{\tclose}{\relax\ifmmode {\sf tclosure} \else ${\sf tclosure}$\fi} 
\newcommand{\card}{\relax\ifmmode {\sf card} \else ${\sf card}$\fi} 
\newcommand{\tabs}[1]{\relax\ifmmode {\sf Untimed}(#1) \else ${\sf TAbs(#1)}$\fi} 

% lstate fstate
\newcommand{\dom}{\relax\ifmmode {\sf dom} \else ${\sf dom}$\fi} 
\newcommand{\lstate}{\relax\ifmmode {\sf lstate} \else ${\sf lstate}$\fi} 
\newcommand{\fstate}{\relax\ifmmode {\sf fstate} \else ${\sf fstate}$\fi} 
\newcommand{\ltime}{\relax\ifmmode {\sf ltime} \else ${\sf ltime}$\fi} 
\newcommand{\prestate}{\relax\ifmmode {\sf prestate} \else ${\sf prestate}$\fi} 
\newcommand{\poststate}{\relax\ifmmode {\sf poststate} \else ${\sf poststate}$\fi} 


\newenvironment{noqedproof}{\pf}{}
\newcommand{\pf}{\par\noindent{\bf Proof:}~}

% repeating theorems: should come after other theorem definitions
\theoremstyle{box}
\newtheorem{duplicate}{NameIgnored}

% ************** Sayan's New definitions will be added in this block END


 %\newtheorem{theorem}{Theorem}[chapter]
% \newtheorem{lem}{Lemma}
 %\newtheorem{corollary}[theorem]{Corollary}
 %\newtheorem{claim}[theorem]{Claim}
%\theoremstyle{definition}
 %\newtheorem{definition}{Definition}[chapter]
 %\renewcommand{\qed}{\hfill{\rule{2mm}{2mm}}\medskip}
 %\newenvironment{proof}{\pf}{\qed}
 %\newtheorem{proposition}[theorem]{Proposition}
%\newenvironment{inv}{\begin{theorem}}{\end{theorem}}
% \newtheorem{inv}{Invariant}
 \newtheorem{assumption}{Assumption}

 
 %\newenvironment{example}
 %{\refstepcounter{theorem} \vspace{2ex}\par\noindent
 %\textbf{Example}~\textbf{\thetheorem~}}{\qed}
 
%\theoremstyle{remark}
% 
% \renewcommand{\theequation}{\thesection.\arabic{equation}}
% \renewcommand{\thefigure}{\thesection.\arabic{figure}}
% \renewcommand{\thetable}{\thesection.\arabic{table}}
% \newcommand{\Section}[1]{\section{#1}%
%    \setcounter{equation}{0}\setcounter{figure}{0}\setcounter{table}{0}%
%    \setcounter{example}{0}}
% 
% \newenvironment{anotation}[1][Nancy]{\begin{quote}\small[[[#1]]]}{\normalsize\end{quote}}
% \newcommand{\ba}{\begin{anotation}}
% \newcommand{\ea}{\end{anotation}}
% 
% \newcommand{\bcb}{\chgbarbegin}
% \newcommand{\ecb}{\chgbarend}
% \chgbarwidth 1pt
% 
% \newcommand{\dec}{\ensuremath{{:}}}
% \newcommand{\eqdef}{\mathbin{::=}}
% \newcommand{\I}{{\ensuremath{\cap}}}



% OPERATIONS ON SETS, RELATIONS AND FUNCTIONS
\newcommand{\pow}[1]{{\bf P}(#1)} % powerset
\newcommand{\inverse}[1]{#1^{-1}}
\newcommand{\range}[1]{\mathit{range{(#1)}}}
\newcommand{\domain}[1]{{\mathit dom}(#1)}
\newcommand{\type}[1]{\mathit{type{(#1)}}}
\newcommand{\val}[1]{\mathit{val{(#1)}}}
\newcommand{\dtype}[1]{\mathit{dtype{(#1)}}} % dynamic type
\newcommand{\restr}{\mathrel{\lceil}}
\newcommand{\proj}{\matrel{\lceil}}
\newcommand{\restrrange}{\mathrel{\downarrow}}
\newcommand{\point}[1]{\wp(#1)}     		%point trajectory



% HYBRID AUTOMATA
\def\A{{\bf A}} % HA
\def\B{{\bf B}} % HA
\def\C{{\cal C}} % HA
\def\D{{\bf D}} % set of discrete steps
\def\DC{{\bf DC}} % points of discontinuity
\def\E{{\cal E}} % HA
\def\F{{\cal F}} % HA
\def\G{{\cal G}} % pieces of SHIOA
\def\H{{\cal H}} % HA
\def\I{{\cal I}} % environment sequence
\def\K{{\cal K}} % environment sequence
\def\M{{\cal M}} % Mode switching transitions
\def\O{{\cal O}} % outcome function
\def\P{{\cal P}} % set of modes
\def\Q{{\cal Q}} % set of modes
\def\R{{\cal R}} % relation
\def\S{{\cal S}} % set of trajectories
\def\T{{\bf T}} % set of trajectories
\def\V{{\cal V}} % Lyapunov function
\def\U{{\cal U}} % set of trajectories
\def\X{{\cal X}} % Lyapunov function
\def\Y{{\cal Y}} % set of trajectories


% more special characters

\newcommand{\col}[1]{\relax\ifmmode \mathscr #1\else $\mathscr #1$\fi}

\def\statemodels{\col{S}}

% LTS related

\newcommand{\atpro}{\mathit{AP}}
\newcommand{\stlab}{\mathit{Lab}}


% Names of actions, automata etc
\definecolor{HIOAcolor}{rgb}{0.776,0.22,0.07}
\newcommand{\HIOA}{\textcolor{HIOAcolor}{\tt HIOA\hspace{3pt}}}
\newcommand{\PVS}{\textcolor{HIOAcolor}{\tt PVS\hspace{3pt}}}
\newcommand{\PVSnogap}{\textcolor{HIOAcolor}{\tt PVS\hspace{1pt}}}
\newcommand{\HIOAbiggap}{\textcolor{HIOAcolor}{\tt HIOA\hspace{6pt}}}
\newcommand{\HIOAnogap}{\textcolor{HIOAcolor}{\tt HIOA}}
\newcommand{\anyrelation}{\lessgtr}


% Transformation for ADT
\newcommand{\SC}[2]{\relax\ifmmode {\tt Scount}(#1,#2) \else ${\tt Scount}(#1,#2)$\fi} 
\newcommand{\SCM}[2]{\relax\ifmmode {\tt Smin}(#1,#2) \else ${\tt Smin}(#1,#2)$\fi} 
\newcommand{\Aut}[1]{\relax\ifmmode {\tt Aut}(#1) \else ${\tt Aut}(#1)$\fi} 

\newcommand{\auto}[1]{{\operatorname{\mathsf{#1}}}}
\newcommand{\act}[1]{{\operatorname{\mathsf{#1}}}}
\newcommand{\smodel}[1]{{\operatorname{\mathsf{#1}}}}
\newcommand{\pvstheory}[1]{{\operatorname{\mathit{#1}}}}
%\newcommand{\auto}[1]{\relax\ifmmode \sf #1\else $\sf #1$\fi}
%\newcommand{\act}[1]{\relax\ifmmode \sf #1\else $\sf #1$\fi}


\newcommand{\Automaton}{{\bf automaton}}
\newcommand{\Asserts}{{\bf asserts}}
\newcommand{\Assumes}{{\bf assumes}}
\newcommand{\Backward}{{\bf backward}}
\newcommand{\By}{{\bf by}}
\newcommand{\Case}{{\bf case}}
\newcommand{\Choose}{{\bf  choose}}
\newcommand{\Components}{{\bf components}}
\newcommand{\Const}{{\bf const}}
\newcommand{\Converts}{{\bf converts}}
\newcommand{\Do}{{\bf do}}
\newcommand{\Eff}{{\bf eff}}
%\newcommand{\Else}{{\bf else}}
\newcommand{\Elseif}{{\bf elseif}}
\newcommand{\Enumeration}{{\bf enumeration}}
\newcommand{\Ensuring}{{\bf ensuring}}
\newcommand{\Exempting}{{\bf exempting}}
\newcommand{\Fi}{{\bf fi}}
%\newcommand{\For}{{\bf for}}
\newcommand{\Forward}{{\bf forward}}
\newcommand{\Freely}{{\bf freely}}
\newcommand{\From}{{\bf from}}
\newcommand{\Generated}{{\bf generated}}
\newcommand{\Local}{{\bf local}}
\newcommand{\Hidden}{{\bf hidden}}
%\newcommand{\If}{{\bf if}}
\newcommand{\In}{{\bf in}}
\newcommand{\Implies}{{\bf implies}}
\newcommand{\Includes}{{\bf includes}}
\newcommand{\Introduces}{{\bf introduces}}
\newcommand{\Input}{{\bf input}}
\newcommand{\Kind}{{\bf kind}}
\newcommand{\Initially}{{\bf initially}}
\newcommand{\Internal}{{\bf internal}}
\newcommand{\Inv}{{\bf invariant}}
\newcommand{\Mode}{{\bf mode}}
\newcommand{\Od}{{\bf od}}
\newcommand{\Of}{{\bf of}}
\newcommand{\Output}{{\bf output}}
\newcommand{\Partitioned}{{\bf partitioned}}
\newcommand{\Pre}{{\bf pre}}
\newcommand{\Signature}{{\bf signature}}
\newcommand{\Simulation}{{\bf simulation}}
\newcommand{\Sort}{{\bf sort}}
\newcommand{\States}{{\bf states}}
\newcommand{\Tasks}{{\bf tasks}}
\newcommand{\Then}{{\bf then}}
\newcommand{\To}{{\bf to}}
\newcommand{\Trait}{{\bf trait}}
\newcommand{\Traits}{{\bf traits}}
\newcommand{\Transitions}{{\bf transitions}}
\newcommand{\Trajectories}{{\bf trajectories}}
\newcommand{\Tuple}{{\bf tuple}}
\newcommand{\Type}{{\bf type}}
\newcommand{\Union}{{\bf union}}
\newcommand{\Uses}{{\bf uses}}
\newcommand{\Var}{{\bf variables}}
\newcommand{\Where}{{\bf where}}
%\newcommand{\While}{{\bf while}}
\newcommand{\With}{{\bf with}}


% Spacing
\newcommand{\FFF}{\vspace{0.1in}}
\newcommand{\BBB}{\hspace{-0.1in}}


\newcommand{\deq}{\mathrel{\stackrel{\scriptscriptstyle\Delta}{=}}}


% systematic labels

\newcommand{\chaplabel}[1]{\label{chap:#1}}
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\chapreftwo}[2]{Chapters~\ref{chap:#1}~and~\ref{chap:#2}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\sseclabel}[1]{\label{subsec:#1}}
\newcommand{\ssecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\secreftwo}[2]{Sections~\ref{sec:#1}~and~\ref{sec:#2}}
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\figrefs}[2]{Figures~\ref{fig:#1} and~\ref{fig:#2}}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\lnlabel}[1]{\label{line:#1}}
\newcommand{\lnrngref}[2]{lines~\ref{line:#1}--\ref{line:#2}\xspace}
\newcommand{\lnref}[1]{line~\ref{line:#1}\xspace}
\newcommand{\lemlabel}[1]{\label{lemma:#1}} 
\newcommand{\lemref}[1]{Lemma~\ref{lemma:#1}\xspace}
\newcommand{\thmlabel}[1]{\label{thm:#1}} 
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}\xspace}
\newcommand{\invlabel}[1]{\label{inv:#1}} 
\newcommand{\invref}[1]{Invariant~\ref{inv:#1}\xspace}
\newcommand{\problemlabel}[1]{\label{problem:#1}} 
\newcommand{\problemref}[1]{Problem~\ref{problem:#1}\xspace}
\newcommand{\deflabel}[1]{\label{def:#1}} 
\newcommand{\defref}[1]{Definition~\ref{def:#1}\xspace}
\newcommand{\exerciselabel}[1]{\label{exer:#1}} 
\newcommand{\exerciseref}[1]{Exercise~\ref{exer:#1}\xspace}
\newcommand{\proplabel}[1]{\label{prop:#1}} 
\newcommand{\propref}[1]{Proposition~\ref{prop:#1}\xspace}

% defs FROM ptioa PAPER


\newcommand{\remove}[1]{}
\newcommand{\salg}[1]{\relax\ifmmode {\mathcal F}_{#1}\else ${\mathcal F}_{#1}$\fi} 
\newcommand{\msp}[1]{\relax\ifmmode (#1, \salg{#1}) \else $(#1, \salg{#1})$\fi} 
\newcommand{\msprod}[2]{\relax\ifmmode ( #1 \times #2, \salg{#1} \otimes \salg{#2}) \else $(#1 \times #2, \salg{#1} \otimes \salg{#2})$\fi} 
\newcommand{\dist}[1]{\relax\ifmmode {\mathcal P}\msp{#1}
  \else ${\mathcal P}\msp{#1}$\fi} 
\newcommand{\subdist}[1]{\relax\ifmmode {\mathcal S}{\mathcal P}\msp{#1} 
  \else ${\mathcal S}{\mathcal P}\msp{#1}$\fi} 
\newcommand{\disc}[1]{\relax\ifmmode {\sf Disc}(#1)
  \else ${\sf Disc}(#1)$\fi} 

\newcommand{\Trajeq}{\relax\ifmmode {\mathcal R}_\T \else ${\mathcal R}_\T$\fi} 
\newcommand{\Acteq}{\relax\ifmmode {\mathcal R}_A \else ${\mathcal R}_A$\fi} 
\newcommand{\noop}{\relax\ifmmode \lambda \else $\lambda$\fi} 
\newcommand{\close}[1]{\relax\ifmmode \overline{#1} \else $\overline{#1}$\fi} 

\newcommand{\corrtasks}{\mathop{\mathsf {c}}}
\newcommand{\full}{\mathop{\mathsf {full}}}
%\newcommand{\fstate}{\mathop{\mathsf {fstate}}}
%\newcommand{\lstate}{\mathop{\mathsf {lstate}}}
\newcommand{\tdist}{\mathop{\mathsf {tdist}}}
\newcommand{\extbeh}{\mathop{\mathsf {extbeh}}}
%\newcommand{\apply}{\mathop{\mathsf {apply}}}
\newcommand{\apply}[2]{\mathop{\mathsf {apply}({#1},{#2})}}
%\newcommand{\applytwo}{\mathop{\mathsf {apply2}}}
\newcommand{\support}{\mathop{\mathsf {supp}}}
\newcommand{\relation}{\mathrel{R}}
\newcommand{\cone}{C}
%\newcommand{\tracef}{\mathord{\mathsf {trace}}}
\newcommand{\flatten}{\mathord{\mathsf {flatten}}}
\newcommand{\discrete}{\mathord{\mathsf {Disc}}}
\newcommand{\lift}[1]{\mathrel{{\mathcal L}(#1)}}
\newcommand{\expansion}[1]{\mathrel{{\mathcal E}(#1)}}
%End of commands added by Roberto on May, 12

%>> Ling, December 2005

\newcommand{\subdisc}{\operatorname{\mathsf {SubDisc}}}
\newcommand{\tran}{\operatorname{\mathsf {tran}}}
%\newcommand{\act}{\operatorname{\mathsf {act}}}

\renewcommand{\execs}{{\operatorname{\mathsf {Execs}}}}
\newcommand{\frags}{{\operatorname{\mathsf {Frags}}}}

\newcommand{\tracefnc}{{\operatorname{\mathsf {trace}}}}
\newcommand{\untimefnc}{{\operatorname{\mathsf {untime}}}}

\newcommand{\finite}{{\operatorname{\mathsf {finite}}}}
\newcommand{\hide}{{\operatorname{\mathsf {hide}}}}

\newcommand{\early}{{\operatorname{\mathsf {Early}}}}
\newcommand{\late}{{\operatorname{\mathsf {Late}}}}
\newcommand{\toss}{{\operatorname{\mathsf {Toss}}}}

\newcommand{\define}{:=}

\newcommand{\pc}{{\operatorname{\mathsf {counter}}}}
\newcommand{\chosen}{{\operatorname{\mathsf {chosen}}}}

\newcommand{\rand}{{\operatorname{\mathsf {random}}}}
\newcommand{\unif}{{\operatorname{\mathsf {unif}}}}

\newcommand{\ie}{i.e.,\xspace}
\newcommand{\Ie}{I.e.,\xspace}

\newcommand{\eg}{e.g.,\xspace}
\newcommand{\Eg}{E.g.,\xspace}

% IOA related stuff




\newcommand{\mybox}[3]{
  \framebox[#1][l]
  {
    \parbox{#2}
    {
      #3
    }
  }
}

\newcommand{\two}[4]{
  \parbox{.95\columnwidth}{\vspace{1pt} \vfill
    \parbox[t]{#1\columnwidth}{#3}%
    \parbox[t]{#2\columnwidth}{#4}%
  }}

\newcommand{\twosep}[4]{
  \parbox{\columnwidth}{\vspace{1pt} \vfill
    \parbox[t]{#1\columnwidth}{#3}%
   	\vrule width 0.2pt
    \parbox[t]{#2\columnwidth}{#4}%
  }}

\newcommand{\eqntwo}[4]{
  \parbox{\columnwidth}{\vspace{1pt} \vfill
    \parbox[t]{#1\columnwidth}{$ #3 $}
    \parbox[t]{#2\columnwidth}{$ #4 $}
  }}

\newcommand{\three}[6]{\vspace{1pt} \vfill
        \parbox{\columnwidth}{%
        \parbox[t]{#1\columnwidth}{#4}%
        \parbox[t]{#2\columnwidth}{#5}%
        \parbox[t]{#3\columnwidth}{#6}%
      }}

\newcommand{\tup}[1]
           {
             \relax\ifmmode
             ( #1 )
             \else $($ #1 $)$ \fi
           }

\newcommand{\lit}[1]{ \relax\ifmmode
                \mathord{\mathcode`\-="702D\sf #1\mathcode`\-="2200}
                \else {\it #1} \fi }


\newcommand{\figuresize}{\scriptsize}

\newcommand{\equationsize}{\footnotesize}

%\newcommand{\act}[1]{%
%  \relax\ifmmode
%                \mathord{\mathcode`\-="702D\sf #1\mathcode`\-="2200}%
%                \else
%                {\sf #1\/}%
%                \fi }


\lstdefinelanguage{ioa}{
  basicstyle=\figuresize,
  keywordstyle=\bf \figuresize,
  identifierstyle=\it \figuresize,
  emphstyle=\tt \figuresize,
  mathescape=true,
  tabsize=20,
%  tabsize=4,
  sensitive=false,
  columns=fullflexible,
  keepspaces=false,
  flexiblecolumns=true,
%  basewidth=0.5em,
  basewidth=0.05em,
  moredelim=[il][\rm]{//},
  moredelim=[is][\sf \figuresize]{!}{!},
  moredelim=[is][\bf \figuresize]{*}{*},
  keywords={automaton, and, actions,
  	 choose,const,continue, components,
  	 discrete, do,
  	 eff, external,else, elseif, evolve, end,
  	 fi,for, forward, from,
  	 hidden,
  	 in,input,internal,if,invariant, initially, imports,
     let,
	mode,
     or, output, operators, od, of,
     pre,
     return,
     such,satisfies, stop, signature, simulation, 
     trajectories,trajdef, transitions, that,then, type, types, to, tasks,
     variables, vocabulary, 
     when,where, with,while},
  emph={set, seq, tuple, map, array, enumeration, powerset},   
   literate=
        {(}{{$($}}1
        {)}{{$)$}}1
        % LaTeX math symbols
        {\\in}{{$\in\ $}}1
        {\\preceq}{{$\preceq\ $}}1
        {\\subset}{{$\subset\ $}}1
        {\\subseteq}{{$\subseteq\ $}}1
        {\\supset}{{$\supset\ $}}1
        {\\supseteq}{{$\supseteq\ $}}1
        {\\forall}{{$\forall$}}1
        {\\le}{{$\le\ $}}1
        {\\ge}{{$\ge\ $}}1
        {\\gets}{{$\gets\ $}}1
        {\\cup}{{$\cup\ $}}1
        {\\cap}{{$\cap\ $}}1
        {\\langle}{{$\langle$}}1
        {\\rangle}{{$\rangle$}}1
        {\\exists}{{$\exists\ $}}1
        {\\bot}{{$\bot$}}1
        {\\rip}{{$\rip$}}1
        {\\emptyset}{{$\emptyset$}}1
        {\\notin}{{$\notin\ $}}1
        {\\not\\exists}{{$\not\exists\ $}}1
        {\\ne}{{$\ne\ $}}1
        {\\to}{{$\to\ $}}1
        {\\implies}{{$\implies\ $}}1
        % LSL symbols (one-character)
        {<}{{$<\ $}}1
        {>}{{$>\ $}}1
        {=}{{$=\ $}}1
        {~}{{$\neg\ $}}1
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall\ $}}1
        {\\E}{{$\exists\ $}}1
        {\\/}{{$\vee\,$}}1
        {\\vee}{{$\vee\,$}}1
        {/\\}{{$\wedge\,$}}1
        {\\wedge}{{$\wedge\,$}}1
        {=>}{{$\Rightarrow\ $}}1
        {->}{{$\rightarrow\ $}}1
        {<=}{{$\Leftarrow\ $}}1
        {<-}{{$\leftarrow\ $}}1
%        {<=}{{$\leq$}}1
%        {>=}{{$\geq$}}1
        {~=}{{$\neq\ $}}1
        {\\U}{{$\cup\ $}}1
        {\\I}{{$\cap\ $}}1
        {|-}{{$\vdash\ $}}1
        {-|}{{$\dashv\ $}}1
        {<<}{{$\ll\ $}}2
        {>>}{{$\gg\ $}}2
        {||}{{$\|$}}1
%%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
%%        {[}{{$\langle$}}1
%%        {]}{{$\rangle$}}1
        {[}{{$[$}}1
        {]}{{$\,]$}}1
        {[[}{{$\langle$}}1
        {]]]}{{$]\rangle$}}1
        {]]}{{$\rangle$}}1
        {<=>}{{$\Leftrightarrow\ $}}2
        {<->}{{$\leftrightarrow\ $}}2
        {(+)}{{$\oplus\ $}}1
        {(-)}{{$\ominus\ $}}1
        {_i}{{$_{i}$}}1
        {_j}{{$_{j}$}}1
        {_{i,j}}{{$_{i,j}$}}3
        {_{j,i}}{{$_{j,i}$}}3
        {_0}{{$_0$}}1
        {_1}{{$_1$}}1
        {_2}{{$_2$}}1
        {_n}{{$_n$}}1
        {_p}{{$_p$}}1
        {_k}{{$_n$}}1
        {-}{{$\ms{-}$}}1
        {@}{{}}0
        {\\delta}{{$\delta$}}1
        {\\R}{{$\R$}}1
        {\\Rplus}{{$\Rplus$}}1
        {\\N}{{$\N$}}1
        {\\times}{{$\times\ $}}1
        {\\tau}{{$\tau$}}1
        {\\alpha}{{$\alpha$}}1
        {\\beta}{{$\beta$}}1
        {\\gamma}{{$\gamma$}}1
        {\\ell}{{$\ell\ $}}1
        {--}{{$-\ $}}1
        {\\TT}{{\hspace{1.5em}}}3        
      }

\lstdefinelanguage{ioaNums}[]{ioa}
{
  numbers=left,
  numberstyle=\tiny,
  stepnumber=2,
  numbersep=4pt
%  firstnumber=1
}

\lstdefinelanguage{ioaNumsRight}[]{ioa}
{
  numbers=right,
  numberstyle=\tiny,
  stepnumber=2,
  numbersep=4pt
%  firstnumber=1
}

\newcommand{\ioa}{\lstinline[language=ioa]}

\lstnewenvironment{IOA}%
  {\lstset{language=IOA}}
  {}

\lstnewenvironment{IOANums}%
  {
  \if@firstcolumn
    \lstset{language=IOA, numbers=left, firstnumber=auto}
  \else
    \lstset{language=IOA, numbers=right, firstnumber=auto}
  \fi
  }
  {}

\lstnewenvironment{IOANumsRight}%
  {
    \lstset{language=IOA, numbers=right, firstnumber=auto}
  }
  {}

%\lstnewenvironment{IOA}%
%  {\lstset{language=ioaLang}
%   \csname lst@SetFirstLabel\endcsname}
%  {\csname lst@SaveFirstLabel\endcsname\vspace{-4pt}\noindent}

\newcommand{\figioa}[5]{
  \begin{figure}[#1]
      \hrule \F
      {\figuresize \bf #2}
      \lstinputlisting[language=ioaLang]{#5}
      \F \hrule \F
      \caption{#3}
      \label{fig: #4}
  \end{figure}
}

\newcommand{\linefigioa}[9]{

}

\newcommand{\twofigioa}[8]{
  \begin{figure}[#1]
    \hrule \F
    {\figuresize \bf #2} \\
    \two{#5}{#6}
    {
      \lstinputlisting[language=ioaLang]{#7}
    }
    {
      \lstinputlisting[language=ioaLang]{#8}
    }
    \F \hrule \F
    \caption{#3}
    \label{fig: #4}
  \end{figure}
}



\lstdefinelanguage{ioaLang}{%
  basicstyle=\ttfamily\small,
  keywordstyle=\rmfamily\bfseries\small,
  identifierstyle=\small,
%  commentline=\%,
  keywords={assumes,automaton,axioms,backward,bounds,by,case,choose,components,const,d,det,discrete,do,eff,else,elseif,ensuring,enumeration,evolve,fi,fire,follow,for,forward,from,hidden,if,in,%
    input,initially,internal,invariant,let, local,model,od,of,output,pre,schedule,signature,so,%
    simulation,states,variables, tasks, stop,tasks,that,then,to,trajdef,trajectory,trajectories,transitions,tuple,type,union,urgent,uses,when,where,while,yield},
  literate=
        % LaTeX math symbols
        {\\in}{{$\in$}}1
        {\\preceq}{{$\preceq$}}1
        {\\subset}{{$\subset$}}1
        {\\subseteq}{{$\subseteq$}}1
        {\\supset}{{$\supset$}}1
        {\\supseteq}{{$\supseteq$}}1
        {\\rho}{{$\rho$}}1
        {\\infty}{{$\infty$}}1
        % LSL symbols (one-character)
        {<}{{$<$}}1
        {>}{{$>$}}1
        {=}{{$=$}}1
        {~}{{$\neg$}}1 
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall$}}1 {\\E}{{$\exists$}}1
        {\\/}{{$\vee$}}1 {/\\}{{$\wedge$}}1 
        {=>}{{$\Rightarrow$}}1 
        {->}{{$\rightarrow$}}1 
        {<=}{{$\leq$}}1 {>=}{{$\geq$}}1 {~=}{{$\neq$}}1
        {\\U}{{$\cup$}}1 {\\I}{{$\cap$}}1
        {|-}{{$\vdash$}}1 {-|}{{$\dashv$}}1
        {<<}{{$\ll$}}2 {>>}{{$\gg$}}2
        {||}{{$\|$}}1
%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
        % LSL symbols (three or more characters)
        {<=>}{{$\Leftrightarrow$}}2 
        {<->}{{$\leftrightarrow$}}2
        {(+)}{{$\oplus$}}1
        {(-)}{{$\ominus$}}1
}

\lstdefinelanguage{bigIOALang}{%
  basicstyle=\ttfamily,
  keywordstyle=\rmfamily\bfseries,
  identifierstyle=,
%  commentline=\%,
  keywords={assumes,automaton,axioms,backward,by,case,choose,components,const,%
    d,det,discrete,do,eff,else,elseif,ensuring,enumeration,evolve,fi,for,forward,from,hidden,if,in%
    input,initially,internal,invariant,mode,local,od,of,output,pre,schedule,signature,so,%
    tasks, simulation,states,stop,tasks,that,then,to,trajdef,trajectories,transitions,tuple,type,union,urgent,uses,when,where,yield},
  literate=
        % LaTeX math symbols
        {\\in}{{$\in$}}1
        {\\preceq}{{$\preceq$}}1
        {\\subset}{{$\subset$}}1
        {\\subseteq}{{$\subseteq$}}1
        {\\supset}{{$\supset$}}1
        {\\supseteq}{{$\supseteq$}}1
        % LSL symbols (one-character)
        {<}{{$<$}}1
        {>}{{$>$}}1
        {=}{{$=$}}1
        {~}{{$\neg$}}1 
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall$}}1 {\\E}{{$\exists$}}1
        {\\/}{{$\vee$}}1 {/\\}{{$\wedge$}}1 
        {=>}{{$\Rightarrow$}}1 
        {->}{{$\rightarrow$}}1 
        {<=}{{$\leq$}}1 {>=}{{$\geq$}}1 {~=}{{$\neq$}}1
        {\\U}{{$\cup$}}1 {\\I}{{$\cap$}}1
        {|-}{{$\vdash$}}1 {-|}{{$\dashv$}}1
        {<<}{{$\ll$}}2 {>>}{{$\gg$}}2
        {||}{{$\|$}}1
%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
        % LSL symbols (three or more characters)
        {<=>}{{$\Leftrightarrow$}}2 
        {<->}{{$\leftrightarrow$}}2
        {(+)}{{$\oplus$}}1
        {(-)}{{$\ominus$}}1
}


\lstnewenvironment{BigIOA}%
  {\lstset{language=bigIOALang,basicstyle=\ttfamily}
   \csname lst@SetFirstLabel\endcsname}
  {\csname lst@SaveFirstLabel\endcsname\vspace{-4pt}\noindent}

\lstnewenvironment{SmallIOA}%
  {\lstset{language=ioaLang,basicstyle=\ttfamily\scriptsize}
   \csname lst@SetFirstLabel\endcsname}
  %{\csname lst@SaveFirstLabel\endcsname\vspace{-4pt}\noindent}
  {\csname lst@SaveFirstLabel\endcsname\noindent}


\newcommand{\true}{\relax\ifmmode \mathit true \else \em true \/\fi}
\newcommand{\false}{\relax\ifmmode \mathit false \else \em false \/\fi}


\newcommand{\Real}{{\operatorname{\texttt{Real}}}}
\newcommand{\Bool}{{\operatorname{\texttt{Bool}}}}
\newcommand{\Char}{{\operatorname{\texttt{Char}}}}
\newcommand{\ioaInt}{{\operatorname{\texttt{Int}}}}
\newcommand{\ioaNat}{{\operatorname{\texttt{Nat}}}}
\newcommand{\ioaAugR}{{\operatorname{\texttt{AugmentedReal}}}}
\newcommand{\ioaString}{{\operatorname{\texttt{String}}}}
\newcommand{\Discrete}{{\operatorname{\texttt{Discrete}}}}
%\newcommand{\Bool}{{\operatorname{\texttt{Bool}}}}

%\newcommand{\lnot}{\neg}
%\newcommand{\land}{\wedge}
%\newcommand{\lor}{\vee}
\newcommand{\limplies}{\Rightarrow}
\newcommand{\liff}{\Leftrightarrow}

\newlength{\bracklen}
\newcommand{\sem}[1]{\settowidth{\bracklen}{[}
     [\hspace{-0.5\bracklen}[#1]\hspace{-0.5\bracklen}]}

\newcommand{\defaultArraystretch}{1.4}
\renewcommand{\arraystretch}{\defaultArraystretch}

\newcommand{\gS}{\mathcal{S}}
\newcommand{\gV}{\mathcal{V}}
\newcommand{\freevars}{\mathcal{FV}}

\newcommand{\gVspec}{\mathcal{V}_\mathit{spec}}
\newcommand{\gVa}{\mathcal{V}_\mathit{A}}
\newcommand{\gVsig}{\mathcal{V}_\mathit{sigs}}
\newcommand{\gVso}{\mathcal{V}_\mathit{sorts}}
\newcommand{\gVop}{\mathcal{V}_\mathit{ops}}
\newcommand{\sort}{\mathit{sort}}
\newcommand{\sig}{\mathit{sig}}
\newcommand{\id}{\mathit{id}}
\newcommand{\sigsep}{\lsl`->`}

%\newcommand{\T}{\mathit{true}}
%\newcommand{\F}{\mathit{false}}

\newcommand{\super}[2]{\ensuremath{\mathit{#1}^\mathit{#2}}}
\newcommand{\tri}[3]{\ensuremath{\mathit{#1}^\mathit{#2}_\mathit{#3}}}
\newcommand{\Assumptions}{\ensuremath{\mathit{Assumptions}}}
\newcommand{\actPred}[3][\pi]{\tri{P}{#2,#1}{#3}}
\newcommand{\actualTypes}[1]{\super{actualTypes}{#1}}
\newcommand{\actuals}[1]{\super{actuals}{#1}}
\newcommand{\autActVars}[2][\pi]{\vars{#2}{},\vars{#2,#1}{}}
\newcommand{\bracket}[2]{\mathit{#1}[\mathit{#2}]}
\newcommand{\compVars}[1]{\super{compVars}{#1}}
\newcommand{\context}{\mathit{context}}
\newcommand{\ensuring}[2]{\tri{ensuring}{#1}{#2}}
\newcommand{\initPred}[1]{\tri{P}{#1}{init}}
\newcommand{\initVals}[1]{\super{initVals}{#1}}
\newcommand{\initially}[2]{\tri{initially}{#1}{#2}}
\newcommand{\invPred}[2]{\tri{Inv}{#1}{#2}}
\newcommand{\knownVars}[1]{\super{knownVars}{#1}}
\newcommand{\localPostVars}[2]{\tri{localPostVars}{#1}{#2}}
\newcommand{\localVars}[2]{\tri{localVars}{#1}{#2}}
\newcommand{\locals}[1]{\bracket{Locals}{#1}}
\newcommand{\nam}[1]{\rho^{\mathit{#1}}}
\newcommand{\otherActPred}[3][\pi]{\otherTri{P}{#2,#1}{#3}}
\newcommand{\otherParams}[2]{\otherTri{params}{#1}{#2}}
\newcommand{\otherSub}[2]{\otherTri{\sigma}{#1}{#2}}
\newcommand{\otherTri}[3]{\tri{\smash{#1'}}{#2}{#3}}
\newcommand{\otherVars}[2]{\otherTri{vars}{#1}{#2}}
\newcommand{\params}[2]{\tri{params}{#1}{#2}}
\newcommand{\postVars}[1]{\super{postVars}{#1}}
\newcommand{\pre}[2]{\tri{Pre}{#1}{#2}}
\newcommand{\prog}[2]{\tri{Prog}{#1}{#2}}
\newcommand{\prov}[2]{\tri{Prov}{#1}{#2}}
\newcommand{\stateSorts}[1]{\super{stateSorts}{#1}}
\newcommand{\stateVars}[1]{\super{stateVars}{#1}}
\newcommand{\states}[1]{\bracket{States}{#1}}
\newcommand{\sub}[2]{\tri{\sigma}{#1}{#2}}
\newcommand{\sugActPred}[3][\pi]{\tri{P}{#2,#1}{#3,desug}}
\newcommand{\sugLocalVars}[2]{\ifthenelse{\equal{}{#2}}%
                             {\tri{localVars}{#1}{desug}}%
                             {\tri{localVars}{#1}{#2,desug}}}
\newcommand{\sugVars}[2]{\ifthenelse{\equal{}{#2}}%
                        {\tri{vars}{#1}{desug}}%
                        {\tri{vars}{#1}{#2,desug}}}
\newcommand{\cVars}[1]{\super{cVars}{#1}}

\newcommand{\vmap}{\dot{\varrho}}
\newcommand{\map}[2]{\tri{\vmap}{#1}{#2}}

\newcommand{\types}[1]{\super{types}{#1}}
\newcommand{\vars}[2]{\tri{vars}{#1}{#2}}

\newcommand{\subActPred}[3][\pi]{\sub{#2,#1}{#3}(\tri{P}{#2,#1}{#3,desug})}
\newcommand{\subLocalVars}[2]{\sub{#1}{#2}(\tri{localVars}{#1}{#2,desug})}

\newcommand{\dA}{\hat{A}}
\newcommand{\renameAction}[1]{\ensuremath{\rho_{#1}(\vars{\dA{#1},\pi}{})}}
\newcommand{\renameComponent}[1]{\ensuremath{\rho_{#1}\dA_{#1}}}

\newenvironment{Syntax}{\[\begin{subSyntax}}{\end{subSyntax}\]\vspace{-.3in}}
\newenvironment{subSyntax}{\begin{array}{l}}{\end{array}}
\newcommand{\w}[1]{\mbox{\hspace*{#1em}}}



%TIOA macros
% Script math symbol name
\newcommand{\ms}[1]{\ifmmode%
\mathord{\mathcode`-="702D\it #1\mathcode`\-="2200}\else%
$\mathord{\mathcode`-="702D\it #1\mathcode`\-="2200}$\fi}

%\newcommand{\domain}[1]{{\it dom}(#1)} % domain

% KEYWORDS 
\newcommand{\kw}[1]{{\bf #1}} 
\newcommand{\tcon}[1]{{\tt #1}} 
\newcommand{\syn}[1]{{\tt #1}} 
\newcommand{\pvskw}[1]{{\sc #1}} 
\newcommand{\pvsid}[1]{{\operatorname{\mathit{#1}}}}


% VALUATIONS
\newcommand{\vv}{{\bf v}}
\newcommand{\vw}{{\bf w}}
\newcommand{\vx}{{\bf x}}
\newcommand{\vy}{{\bf y}}
\newcommand{\va}{{\bf a}}
\newcommand{\vb}{{\bf b}}
\newcommand{\vg}{\mathit{g}}
\newcommand{\vq}{{\bf q}}
\newcommand{\vs}{{\bf s}}
\newcommand{\vm}{{\bf m}}

% Transitions and trajectory operations
\newcommand{\arrow}[1]{\mathrel{\stackrel{#1}{\rightarrow}}}
\newcommand{\sarrow}[2]{\mathrel{\stackrel{#1}{\rightarrow_{#2}}}}
\newcommand{\concat}{\mathbin{^{\frown}}} % concatenation
\newcommand{\paste}{\mathrel{\diamond}}
\newcommand{\sembrack}[1]{[\![#1]\!]}

\newcommand{\groupop}{\circ}

\def\CC{{\mathscr C}} % concatenation closure

% PVS STUFF

\lstdefinelanguage{pvs}{
  basicstyle=\tt \figuresize,
  keywordstyle=\sc \figuresize,
  identifierstyle=\it \figuresize,
  emphstyle=\tt \figuresize,
  mathescape=true,
  tabsize=20,
%  tabsize=4,
  sensitive=false,
  columns=fullflexible,
  keepspaces=false,
  flexiblecolumns=true,
%  basewidth=0.5em,
  basewidth=0.05em,
  moredelim=[il][\rm]{//},
  moredelim=[is][\sf \figuresize]{!}{!},
  moredelim=[is][\bf \figuresize]{*}{*},
  keywords={and, 
  	 begin,
  	 cases, const,
  	 do,
  	 external, else, exists, end, endcases, endif,
  	 fi,for, forall, from,
  	 hidden,
  	 in, if, importing,
     let, lambda, lemma,
     measure, 
     not,
     or, of,
     return, recursive,
     stop, 
     theory, that,then, type, types, type+, to, theorem,
     var,
     with,while},
  emph={nat, setof, sequence, eq, tuple, map, array, enumeration, bool, real, exp, nnreal, posreal},   
   literate=
        {(}{{$($}}1
        {)}{{$)$}}1
        % LaTeX math symbols
        {\\in}{{$\in\ $}}1
        {\\mapsto}{{$\rightarrow\ $}}1
        {\\preceq}{{$\preceq\ $}}1
        {\\subset}{{$\subset\ $}}1
        {\\subseteq}{{$\subseteq\ $}}1
        {\\supset}{{$\supset\ $}}1
        {\\supseteq}{{$\supseteq\ $}}1
        {\\forall}{{$\forall$}}1
        {\\le}{{$\le\ $}}1
        {\\ge}{{$\ge\ $}}1
        {\\gets}{{$\gets\ $}}1
        {\\cup}{{$\cup\ $}}1
        {\\cap}{{$\cap\ $}}1
        {\\langle}{{$\langle$}}1
        {\\rangle}{{$\rangle$}}1
        {\\exists}{{$\exists\ $}}1
        {\\bot}{{$\bot$}}1
        {\\rip}{{$\rip$}}1
        {\\emptyset}{{$\emptyset$}}1
        {\\notin}{{$\notin\ $}}1
        {\\not\\exists}{{$\not\exists\ $}}1
        {\\ne}{{$\ne\ $}}1
        {\\to}{{$\to\ $}}1
        {\\implies}{{$\implies\ $}}1
        % LSL symbols (one-character)
        {<}{{$<\ $}}1
        {>}{{$>\ $}}1
        {=}{{$=\ $}}1
        {~}{{$\neg\ $}}1
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall\ $}}1
        {\\E}{{$\exists\ $}}1
        {\\/}{{$\vee\,$}}1
        {\\vee}{{$\vee\,$}}1
        {/\\}{{$\wedge\,$}}1
        {\\wedge}{{$\wedge\,$}}1
        {->}{{$\rightarrow\ $}}1
        {=>}{{$\Rightarrow\ $}}1
        {->}{{$\rightarrow\ $}}1
        {<=}{{$\Leftarrow\ $}}1
        {<-}{{$\leftarrow\ $}}1
%        {<=}{{$\leq$}}1
%        {>=}{{$\geq$}}1
        {~=}{{$\neq\ $}}1
        {\\U}{{$\cup\ $}}1
        {\\I}{{$\cap\ $}}1
        {|-}{{$\vdash\ $}}1
        {-|}{{$\dashv\ $}}1
        {<<}{{$\ll\ $}}2
        {>>}{{$\gg\ $}}2
        {||}{{$\|$}}1
%%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
%%        {[}{{$\langle$}}1
%%        {]}{{$\rangle$}}1
        {[}{{$[$}}1
        {]}{{$\,]$}}1
        {[[}{{$\langle$}}1
        {]]]}{{$]\rangle$}}1
        {]]}{{$\rangle$}}1
        {<=>}{{$\Leftrightarrow\ $}}2
        {<->}{{$\leftrightarrow\ $}}2
        {(+)}{{$\oplus\ $}}1
        {(-)}{{$\ominus\ $}}1
        {_i}{{$_{i}$}}1
        {_j}{{$_{j}$}}1
        {_{i,j}}{{$_{i,j}$}}3
        {_{j,i}}{{$_{j,i}$}}3
        {_0}{{$_0$}}1
        {_1}{{$_1$}}1
        {_2}{{$_2$}}1
        {_n}{{$_n$}}1
        {_p}{{$_p$}}1
        {_k}{{$_n$}}1
        {-}{{$\ms{-}$}}1
        {@}{{}}0
        {\\delta}{{$\delta$}}1
        {\\R}{{$\R$}}1
        {\\Rplus}{{$\Rplus$}}1
        {\\N}{{$\N$}}1
        {\\times}{{$\times\ $}}1
        {\\tau}{{$\tau$}}1
        {\\alpha}{{$\alpha$}}1
        {\\beta}{{$\beta$}}1
        {\\gamma}{{$\gamma$}}1
        {\\ell}{{$\ell\ $}}1
        {--}{{$-\ $}}1
        {\\TT}{{\hspace{1.5em}}}3        
      }



\lstdefinelanguage{BigPVS}{
  basicstyle=\tt,
  keywordstyle=\sc,
  identifierstyle=\it,
  emphstyle=\tt ,
  mathescape=true,
  tabsize=20,
%  tabsize=4,
  sensitive=false,
  columns=fullflexible,
  keepspaces=false,
  flexiblecolumns=true,
%  basewidth=0.5em,
  basewidth=0.05em,
  moredelim=[il][\rm]{//},
  moredelim=[is][\sf \figuresize]{!}{!},
  moredelim=[is][\bf \figuresize]{*}{*},
  keywords={and, 
  	 begin,
  	 cases, const,
  	 do, datatype,
  	 external, else, exists, end, endif, endcases,
  	 fi,for, forall, from,
  	 hidden,
  	 in, if, importing,
     let, lambda, lemma,
     measure,
     not,
     or, of,
     return, recursive,
     stop, 
     theory, that,then, type, types, type+, to, theorem,
     var,
     with,while},
  emph={nat, setof, sequence, eq, tuple, map, array, first, rest, add, enumeration, bool, real, posreal, nnreal},   
   literate=
        {(}{{$($}}1
        {)}{{$)$}}1
        % LaTeX math symbols
        {\\in}{{$\in\ $}}1
        {\\mapsto}{{$\rightarrow\ $}}1
        {\\preceq}{{$\preceq\ $}}1
        {\\subset}{{$\subset\ $}}1
        {\\subseteq}{{$\subseteq\ $}}1
        {\\supset}{{$\supset\ $}}1
        {\\supseteq}{{$\supseteq\ $}}1
        {\\forall}{{$\forall$}}1
        {\\le}{{$\le\ $}}1
        {\\ge}{{$\ge\ $}}1
        {\\gets}{{$\gets\ $}}1
        {\\cup}{{$\cup\ $}}1
        {\\cap}{{$\cap\ $}}1
        {\\langle}{{$\langle$}}1
        {\\rangle}{{$\rangle$}}1
        {\\exists}{{$\exists\ $}}1
        {\\bot}{{$\bot$}}1
        {\\rip}{{$\rip$}}1
        {\\emptyset}{{$\emptyset$}}1
        {\\notin}{{$\notin\ $}}1
        {\\not\\exists}{{$\not\exists\ $}}1
        {\\ne}{{$\ne\ $}}1
        {\\to}{{$\to\ $}}1
        {\\implies}{{$\implies\ $}}1
        % LSL symbols (one-character)
        {<}{{$<\ $}}1
        {>}{{$>\ $}}1
        {=}{{$=\ $}}1
        {~}{{$\neg\ $}}1
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall\ $}}1
        {\\E}{{$\exists\ $}}1
        {\\/}{{$\vee\,$}}1
        {\\vee}{{$\vee\,$}}1
        {/\\}{{$\wedge\,$}}1
        {\\wedge}{{$\wedge\,$}}1
        {->}{{$\rightarrow\ $}}1
        {=>}{{$\Rightarrow\ $}}1
        {->}{{$\rightarrow\ $}}1
        {<=}{{$\Leftarrow\ $}}1
        {<-}{{$\leftarrow\ $}}1
%        {<=}{{$\leq$}}1
%        {>=}{{$\geq$}}1
        {~=}{{$\neq\ $}}1
        {\\U}{{$\cup\ $}}1
        {\\I}{{$\cap\ $}}1
        {|-}{{$\vdash\ $}}1
        {-|}{{$\dashv\ $}}1
        {<<}{{$\ll\ $}}2
        {>>}{{$\gg\ $}}2
        {||}{{$\|$}}1
%%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
%%        {[}{{$\langle$}}1
%%        {]}{{$\rangle$}}1
        {[}{{$[$}}1
        {]}{{$\,]$}}1
        {[[}{{$\langle$}}1
        {]]]}{{$]\rangle$}}1
        {]]}{{$\rangle$}}1
        {<=>}{{$\Leftrightarrow\ $}}2
        {<->}{{$\leftrightarrow\ $}}2
        {(+)}{{$\oplus\ $}}1
        {(-)}{{$\ominus\ $}}1
        {_i}{{$_{i}$}}1
        {_j}{{$_{j}$}}1
        {_{i,j}}{{$_{i,j}$}}3
        {_{j,i}}{{$_{j,i}$}}3
        {_0}{{$_0$}}1
        {_1}{{$_1$}}1
        {_2}{{$_2$}}1
        {_n}{{$_n$}}1
        {_p}{{$_p$}}1
        {_k}{{$_n$}}1
        {-}{{$\ms{-}$}}1
        {@}{{}}0
        {\\delta}{{$\delta$}}1
        {\\R}{{$\R$}}1
        {\\Rplus}{{$\Rplus$}}1
        {\\N}{{$\N$}}1
        {\\times}{{$\times\ $}}1
        {\\tau}{{$\tau$}}1
        {\\alpha}{{$\alpha$}}1
        {\\beta}{{$\beta$}}1
        {\\gamma}{{$\gamma$}}1
        {\\ell}{{$\ell\ $}}1
        {--}{{$-\ $}}1
        {\\TT}{{\hspace{1.5em}}}3        
      }

\lstdefinelanguage{pvsNums}[]{pvs}
{
  numbers=left,
  numberstyle=\tiny,
  stepnumber=2,
  numbersep=4pt
%  firstnumber=1
}

\lstdefinelanguage{pvsNumsRight}[]{pvs}
{
  numbers=right,
  numberstyle=\tiny,
  stepnumber=2,
  numbersep=4pt
%  firstnumber=1
}

\newcommand{\pvs}{\lstinline[language=PVS]}

\lstnewenvironment{BigPVS}%
  {\lstset{language=BigPVS}}
  {}

\lstnewenvironment{PVSNums}%
  {
  \if@firstcolumn
    \lstset{language=pvs, numbers=left, firstnumber=auto}
  \else
    \lstset{language=pvs, numbers=right, firstnumber=auto}
  \fi
  }
  {}

\lstnewenvironment{PVSNumsRight}%
  {
    \lstset{language=pvs, numbers=right, firstnumber=auto}
  }
  {}


\newcommand{\figpvs}[5]{
  \begin{figure}[#1]
      \hrule \F
      {\figuresize \bf #2}
      \lstinputlisting[language=pvs]{#5}
      \F \hrule \F
      \caption{#3}
      \label{fig: #4}
  \end{figure}
}

\newcommand{\linefigpvs}[9]{

}

\newcommand{\twofigpvs}[8]{
  \begin{figure}[#1]
    \hrule \F
    {\figuresize \bf #2} \\
    \two{#5}{#6}
    {
      \lstinputlisting[language=pvsLang]{#7}
    }
    {
      \lstinputlisting[language=pvsLang]{#8}
    }
    \F \hrule \F
    \caption{#3}
    \label{fig: #4}
  \end{figure}
}


\lstdefinelanguage{pvsproof}{
  basicstyle=\tt \figuresize,
  mathescape=true,
  tabsize=4,
  sensitive=false,
  columns=fullflexible,
  keepspaces=false,
  flexiblecolumns=true,
  basewidth=0.05em,
}


\lstdefinelanguage{pseudocode}{
%	basicstyle=\figuresize,
%	keywordstyle=\bf \figuresize,
%	identifierstyle=\it \figuresize,
%	emphstyle=\tt \figuresize,
	mathescape=true,
	tabsize=20,
	xleftmargin=4.0ex,
	basicstyle=\normalsize,
	sensitive=false,
	columns=fullflexible,
	keepspaces=false,
	%flexiblecolumns=true,
	%  basewidth=0.5em,
	basewidth=0.05em,
	moredelim=[il][\rm]{//},
	moredelim=[is][\sf \figuresize]{!}{!},
	moredelim=[is][\bf \figuresize]{*}{*},
	keywords={automaton, algorithm, and, 
		choose,const,continue, components,
		discrete, do,
		eff, external,else, elseif, evolve, end, each, exit,
		fi,for, forward, from, find, 
		hidden,
		in,input,internal,if,invariant, initially, imports,
		let,
		mode,
		or, output, operators, od, of,
		pre,
		return,
		such,satisfies, stop, signature, simulation, sample,
		trajectories,trajdef, transitions, that,then, type, types, to, tasks,
		variables, vocabulary, 
		when,where, with,while},
	emph={set, seq, tuple, map, array, enumeration},   
	literate=
	{(}{{$($}}1
	{)}{{$)$}}1
	% LaTeX math symbols
	{\\in}{{$\in\ $}}1
	{\\preceq}{{$\preceq\ $}}1
	{\\subset}{{$\subset\ $}}1
	{\\subseteq}{{$\subseteq\ $}}1
	{\\supset}{{$\supset\ $}}1
	{\\supseteq}{{$\supseteq\ $}}1
	{\\forall}{{$\forall$}}1
	{\\le}{{$\le\ $}}1
	{\\ge}{{$\ge\ $}}1
	{\\gets}{{$\gets\ $}}1
	{\\cup}{{$\cup\ $}}1
	{\\cap}{{$\cap\ $}}1
	{\\langle}{{$\langle$}}1
	{\\rangle}{{$\rangle$}}1
	{\\exists}{{$\exists\ $}}1
	{\\bot}{{$\bot$}}1
	{\\rip}{{$\rip$}}1
	{\\emptyset}{{$\emptyset$}}1
	{\\notin}{{$\notin\ $}}1
	{\\not\\exists}{{$\not\exists\ $}}1
	{\\ne}{{$\ne\ $}}1
	{\\to}{{$\to\ $}}1
	{\\implies}{{$\implies\ $}}1
	% LSL symbols (one-character)
	{<}{{$<\ $}}1
	{>}{{$>\ $}}1
	{=}{{$=\ $}}1
	{~}{{$\neg\ $}}1
	{|}{{$\mid$}}1
	{'}{{$^\prime$}}1
	% LSL symbols (two characters)
	{\\A}{{$\forall\ $}}1
	{\\E}{{$\exists\ $}}1
	{\\/}{{$\vee\,$}}1
	{\\vee}{{$\vee\,$}}1
	{/\\}{{$\wedge\,$}}1
	{\\wedge}{{$\wedge\,$}}1
	{=>}{{$\Rightarrow\ $}}1
	{->}{{$\rightarrow\ $}}1
	{<=}{{$\Leftarrow\ $}}1
	{<-}{{$\leftarrow\ $}}1
	%        {<=}{{$\leq$}}1
	%        {>=}{{$\geq$}}1
	{~=}{{$\neq\ $}}1
	{\\U}{{$\cup\ $}}1
	{\\I}{{$\cap\ $}}1
	{|-}{{$\vdash\ $}}1
	{-|}{{$\dashv\ $}}1
	{<<}{{$\ll\ $}}2
	{>>}{{$\gg\ $}}2
	{||}{{$\|$}}1
	%%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
	%%        {[}{{$\langle$}}1
	%%        {]}{{$\rangle$}}1
	{[}{{$[$}}1
	{]}{{$\,]$}}1
	{[[}{{$\langle$}}1
	{]]]}{{$]\rangle$}}1
	{]]}{{$\rangle$}}1
	{<=>}{{$\Leftrightarrow\ $}}2
	{<->}{{$\leftrightarrow\ $}}2
	{(+)}{{$\oplus\ $}}1
	{(-)}{{$\ominus\ $}}1
	{_i}{{$_{i}$}}1
	{_j}{{$_{j}$}}1
	{_{i,j}}{{$_{i,j}$}}3
	{_{j,i}}{{$_{j,i}$}}3
	{_0}{{$_0$}}1
	{_1}{{$_1$}}1
	{_2}{{$_2$}}1
	{_n}{{$_n$}}1
	{_p}{{$_p$}}1
	{_k}{{$_n$}}1
	{-}{{$\ms{-}$}}1
	{@}{{}}0
	{\\delta}{{$\delta$}}1
	{\\R}{{$\R$}}1
	{\\Rplus}{{$\Rplus$}}1
	{\\N}{{$\N$}}1
	{\\times}{{$\times\ $}}1
	{\\tau}{{$\tau$}}1
	{\\alpha}{{$\alpha$}}1
	{\\beta}{{$\beta$}}1
	{\\gamma}{{$\gamma$}}1
	{\\ell}{{$\ell\ $}}1
%	{--}{{$-\ $}}1
	{\\TT}{{\hspace{1.5em}}}3        
}

\lstdefinelanguage{pseudocodeNums}[]{pseudocode}
{
	numbers=left,
	numberstyle=\tiny,
	stepnumber=2,
	numbersep=4pt
	%  firstnumber=1
}

%%%%%%% Mahesh's macros
%
% Turing machine related macros
%
\newcommand{\blank} {\sqcup} %Blank symbol
\newcommand{\leftendmarker} {\rhd} %Left end marker of TM tape
\newcommand{\lft} {\mathsf{L}} %Left direction
\newcommand{\rght} {\mathsf{R}} %Right direction
\newcommand{\qacc} {q_{\mathsf{acc}}} %Accepting state
\newcommand{\qrej} {q_{\mathsf{rej}}} %Rejecting state
\newcommand{\movetm} {\vdash} %Single move of TM
\newcommand{\movetmst} {{\movetm}^*} %Zero or more moves of TM
\newcommand{\tmcode}[1] {\langle #1 \rangle} %Code of a TM

%%% Simulation driven verification related macros
\newcommand{\interval}{\mathit{interval}} %Code of a TM
\newcommand{\ct}{\mathit{center}} %Code of a TM
\newcommand{\rg}{\mathit{range}} %Code of a TM
\newcommand{\vertex} {\mathit{vertex}} %Code of a TM
\newcommand{\dur}{\mathit{dur}} %Code of a TM
\newcommand{\traj}{\mathit{Traj}} %Code of a TM
\newcommand{\Reach}{\mathit{Reach}} %Code of a TM
\newcommand{\gammahat}{\hat{\gamma}} %Code of a TM
\newcommand{\ldfmnorm}{\mathit{ldfnorm}} %Code of a TM
\newcommand{\Loc}{\mathit{Loc}} %Code of a TM
\newcommand{\Vertex}{{\bf V}} %Code of a TM
\newcommand{\Edge}{{\bf E}} %Code of a TM
\newcommand{\elab}{\mathit{elab}} %Code of a TM
\newcommand{\loc}{\mathit{loc}} %Code of a TM
\newcommand{\trajlab}{{\bf TL}} %Code of a TM
\newcommand{\hs}{\mathit{hs}} %Code of a TM
\newcommand{\init}{\mathit{init}} %Code of a TM
\newcommand{\locinit}{\mathit{locinit}} %Code of a TM
\newcommand{\invariant}{\mathit{invariant}} %Code of a TM
\newcommand{\linit}{\mathit{linit}} %Code of a TM
\newcommand{\Lmode}{\mathit{Lmode}} %Code of a TM
\newcommand{\Execs}{\mathit{Execs}} %Code of a TM
\newcommand{\nextInit}{\mathit{nextInit}} %Code of a TM
\newcommand{\remainTime}{\mathit{tRemain}} %Code of a TM
\newcommand{\simulator}{\mathit{sim}} %Code of a TM
\newcommand{\TB}{\mathit{reachtube}} %safe-reachtube output
\newcommand{\findldf}{\sf{compLDF}} 
\newcommand{\coverstack}{\mathit{coverstack}} 
\newcommand{\Rtube}{\mathit{Rtube}} 
\newcommand{\unsafe}{\bf{U}} %Unsafe set
\newcommand{\intA}{\bf{IntA}} %Interval matrix A
\newcommand{\argmin}[1]{\sf{argmin}_{#1}} %Unsafe set
\newcommand{\InitialQueue}{\mathit{queue}} %initial queue
\newcommand{\reachHybrid}{\mathit{reachtube}} %initial queue

\newcommand{\cachTree}{\mathit{cachetree}}
\newcommand{\rootnode}{\mathit{root}} 
\newcommand{\traversalstack}{\mathit{traversalQueue}} 
\newcommand{\node}{\mathit{node}}
\newcommand{\nodechildren}{\mathit{children}}
\newcommand{\initialset}{\mathit{initset}}
\newcommand{\reachset}{\mathit{Reach}} 
\newcommand{\originalalgo}{\mathit{original}}
\newcommand{\supportalgo}{\mathit{support}}  
\newcommand{\overrt}{\mathit{rt}}

==> sayan-prelim.tex <==
\section{Preliminaries}
\label{sec:prelim}

==> sim_driven_verif.tex <==
\subsection{Data-driven verification}
\label{sec:simVerif}
Data-driven verification algorithms  answer the bounded safety verification question using numerical simulation data, that is, samples of the solution $\xi(x_0,t)$.  The key idea is to generalize an individual simulation $\xi(x_0,\cdot)$ to over-approximate the reachtube $\Rtube(B(x_0,\delta),T)$, for some $\delta > 0$. This generalization  covers a $\delta$-ball $B(x_0,\delta)$ of the initial set $K$, and  several simulations can then cover all of $K$ and over-approximate $\Rtube(K,T)$, which in turn could prove safety. If the over-approximations turn out to be too conservative and safety cannot be concluded, then $\delta$ has to be reduced, and more precise over-approximations of $\Rtube(K,T)$ have to be computed with smaller generalization radius $\delta$ and more simulation data. 

Thus far, the generalization strategy has been entirely based on computing sensitivity of the solution $\xi(x_0, t)$ to the initial condition $x_0$. Algorithms have been developed for computing this sensitivity for linear,  nonlinear, and hybrid dynamical models~\cite{breachAD,FanM15:ATVA,FanQM0D16} as well as for estimating sensitivity from black-box systems~\cite{FanQMV:CAV2017}.  The resulting software tools have been successfully applied to  verify  automotive, aerospace, and medical embedded systems~\cite{FanQM18,HuangFMMK14,Prabhakar2015}.


%make this decision using numerical solutions of the ODE system and  {\em sensitivity-analysis\/} of $f$. For the research reported here, we will use the data-driven verification tool C2E2~\cite{FanQM0D16} developed at Illinois. C2E2 computes precise sensitivity functions (formally  {\em discrepancy functions\/}) based on the system model $f$ using the algorithms in~\cite{FanM15:ATVA}. 

 The precise notion of sensitivity needed for the verification algorithm to have soundness and relative completeness is formalized as {\em discrepancy function\/}~\cite{DMVemsoft2013}. 
\begin{definition}
	\label{def:discrepancy}
A discrepancy function of system~(\ref{eq:goal_ode}) with initial set of states $K \subseteq \mathbb{R}^n$ is a class-$\mathcal{K}$ function in the first argument $\beta: \nnreals \times \nnreals \rightarrow \nnreals$ that satisfies the following conditions:
%\begin{inparaenum}
(1) $\forall \ x, x' \in K, t \geq 0$,  
$\|\xi(x,t) - \xi(x',t)\| \leq \beta(\|x - x'\|,t)$,
(2) $\beta(\|\xi(x,t) -\xi(x',t)\|,t) \rightarrow 0$ as $\|x - x'\| \rightarrow 0$.
%\end{inparaenum}
\end{definition}

The first condition in Definition~\ref{def:discrepancy} says that $\beta$ upper-bounds the distance between two trajectories as a function of the distance between their initial states. The second condition makes the bound shrink as the initial states get closer.% There are several methods to compute a discrepancy function using incremental Lyapunov function \cite{Girard2010}, maximal eigenvalues of the Jacobian matrix~\cite{} 
%Thus, as the radius $\delta$  of the partition of the initial set reduces, the over-approximation given by discrepancy function goes down to zero. 
 
Algorithm~\ref{code:safetyVerifAlgo} without the boxed parts describes data-driven verification for a dynamical system~(\ref{eq:goal_ode}). We refer to this algorithm as  $\simVerif$ in this paper. Given the compact initial set of states $K \subseteq \reals^n$, a time bound $T > 0$, and an unsafe set $U$, $\simVerif$ answers the safety verification question. It initializes a stack called $\coverstack$ with a cover of $K$. Then, it checks the safety from each element in  the cover. For a given $B(x_0,\delta)$ in $\coverstack$, $\simVerif$ simulates~(\ref{eq:goal_ode}) from $x_0$ and bloats to compute an over-approximation of $\Rtube(B(x_0,\delta),T)$. Formally, the set $\mathit{sim} \oplus \beta$ is a Minkowski sum. This can be computed by increasing the radius in each dimension of $\mathit{sim}$ at a time instant $t$ by $\beta(\delta, t)$. The first condition on $\beta$ ensures that this set is indeed an over-approximation of $\Rtube(B(x_0,\delta),T)$.
%
If this over-approximation is disjoint from $U$ then it is safe and is removed from $\coverstack$. If instead, the over-approximation intersects with $U$ then that is inconclusive and  $B(x_0,\delta)$ is partitioned into smaller sets and added to $\coverstack$. The second condition on $\beta$ ensures that this {\em refinement\/} leads to a more precise over-approximation of $B(x_0,\delta)$. 
%
On the other hand, if the simulation hits $U$, that serves as  a counterexample and $\simVerif$  returns unsafe. %it cannot decide if it intersects it because of an actual trajectory starting from $K$ or because of the overapproximation error. 
Finally, if $\coverstack$ becomes empty, that implies that the algorithm reached a partition of $K$ from which all the over-approximated reachtubes are disjoint from $U$, and then $\simVerif$ returns safe.
\begin{algorithm}
	\small
	\caption{$\simVerif$ safety verification algorithm}
		\label{code:safetyVerifAlgo}
%\begin{algorithm}	
	\begin{algorithmic}[1]
		\State \textbf{input:} $K, T, U, \Gamma, \beta$
		\State $\coverstack \gets$ finite cover $ \cup_i B(x_i,\delta) \supseteq K$
		\State \tikzmark{startsym1} $\cachTree \gets \emptyset$ \tikzmark{endsym1} \label{ln:initcahcetree}
		\While{$\coverstack \neq \emptyset$}
		\State $B(x_0,\delta) = \coverstack.pop()$
		%\State $\coverstack \gets \coverstack \textbackslash \{B(x_0,\delta)\}$
		\State \tikzmark{startsym}$ ans \gets {\sf{SymmetryandRefine}}(U,\Gamma, \cachTree,B(x_0,\delta))$ \label{ln:symmetrycall}
		\If{$ans = {\sf{Unsafe}}$} 
		\textbf{return:} $ans$
		\ElsIf{$ ans = {\sf{Safe}}$}
		 \textbf{continue} 
		\Else \tikzmark{endsym}\label{ln:endSymBlock}
		\State $\mathit{sim} \gets $simulate  $\xi(x_0,\cdot)$ upto time $T$ \label{ln:sim}
		\State $rt \gets  \mathit{sim} \oplus \beta$ \label{ln:rt}
		\State \tikzmark{startsym2} $\cachTree.insert(node(rt,sim))$\tikzmark{endsym2} \label{ln:addNodeTree} 
		\If{$\mathit{sim}$ intersects with $U$ } 
		\State \textbf{return:} {\sf{Unsafe}}
		\ElsIf{$rt$ intersects with $U$}
		 \State Refine cover and add to the $\coverstack$
		\EndIf
		\EndIf
		\EndWhile
		\State \textbf{return:} {\sf{Safe}}
	\end{algorithmic}
%
\Textbox{startsym1}{endsym1}{}
\Textbox[6.25cm]{startsym}{endsym}{}
\Textbox{startsym2}{endsym2}{}
\end{algorithm}



%\sayan{What is the difference between $\beta$ and $\gamma$?}



%Soundness and relative completeness.



==> sym_ode.tex <==
\subsection{Symmetry in dynamical systems}
\label{sec:symODE}

Symmetry takes a central place in analysis of dynamical systems~\cite{Marsden:2010:IMS:1965128}. The research line pertinent to our work develops the conditions under which one can get a solution by transforming another solution~\cite{MarsdenRatiu2010,Olver1986,freund_1986}. First, recall the definition of a group.

\begin{definition} A group $(\Gamma,\groupop)$ is a set $\Gamma$ and an operator $\groupop:\Gamma \times \Gamma \rightarrow \Gamma$ satisfying:
\begin{itemize}
\item Closure: For any $\gamma_1, \gamma_2 \in \Gamma$, $\gamma_1 \groupop \gamma_2 \in \Gamma$
\item Associativity: For any $\gamma_1,\gamma_2,\gamma_3 \in \Gamma$, $\gamma_1 \groupop (\gamma_2 \groupop \gamma_3) = (\gamma_1 \groupop \gamma_2 ) \groupop \gamma_3$.
\item Identity: There is an element $e \in \Gamma$ such that $e \groupop \gamma = \gamma \groupop e = \gamma$.
\item Inverse: For every element $\gamma \in \Gamma$, there exists a unique element $\gamma^{-1} \in \Gamma$, called its inverse, such that $\gamma \groupop \gamma^{-1} =  \gamma^{-1} \groupop \gamma = e$.
\end{itemize}
\end{definition}
%\vspace{-.1in}
Symmetries of dynamical systems are modeled as groups of operators on the state space. 
\vspace{-.1in}
%We now define symmetry in dynamical systems.
\begin{definition}[Definition 2 in \cite{russo2011symmetries}]
	\label{def:symmetry}
	Let $\Gamma$ be a group of operators acting on $\mathbb{R}^n$. We say that $\gamma \in \Gamma$ is a symmetry of (\ref{eq:goal_ode}) if for any solution, $\xi(x_0,t)$, $\gamma \cdot \xi(x_0,t)$ is also a solution. Furthermore, if $\gamma \cdot \xi = \xi$, we say that the solution $\xi$ is $\gamma$-symmetric.
\end{definition}
%\vspace{-.1in}
Thus, if $\gamma$ is a symmetry for (\ref{eq:goal_ode}), then new solutions can be obtained by just applying $\gamma$ to existing solutions. Herein lies the opportunity of exploiting symmetries in data-driven verification. 

How can we know that $\gamma$ is a symmetry for (\ref{eq:goal_ode})? 
It turns out that, a sufficient condition exists that  can be checked without finding the solutions (potentially hard problem), but only by checking commutativity of $\gamma$ with the dynamic function $f$. Systems that meet this criterion are called {\em equivariant}. 



\begin{definition} [Definition 3 in \cite{russo2011symmetries}]
	\label{def:equivariance}
	Let $\Gamma$ be a group of operators acting on $\reals^n$. The dynamic function (vector field) $f: \reals^n \rightarrow \reals^n$  is said to be {\em $\Gamma$-equivariant\/} if $f(\gamma (x)) = \gamma (f(x))$, for any $\gamma \in \Gamma$ and $x \in \reals^n$.
\end{definition}

The following theorem shows that for equivariant systems, solutions are symmetric. 
\begin{theorem}[\cite{golubitsky2012symmetry,russo2011symmetries}]
	\label{thm:sol_transform}
	If~(\ref{eq:goal_ode}) is $\Gamma$-equivariant and $\xi$ is a solution, then so is $\gamma \cdot \xi$, $\forall \gamma \in \Gamma$.
\end{theorem}
\vspace{-.2in}
\section{Symmetries in cyber-physical systems}
\label{sec:symmetry:cps}
\vspace{-.1in}
 Equivariant systems are ubiquitous in nature and in relevant models of cyber-physical systems. Below are few examples of simple equivariant systems with respect to different symmetries. We start with a simple 2-dimensional linear system.

%\sayan{Can we make this a little more interesting? Maybe a diagonal system? scaling + translation together? Why starting with Example 2?}
\begin{example}
	Consider the system 
	\begin{align}
	\label{eq:simplelinear}
	\dot{x}_1 = - x_2, \dot{x}_2 = x_1.
	\end{align}
	where $x_1, x_2 \in \mathbb{R}$.
	Let $\Gamma$ be the set of matrices of the form: 
	$B = [[a,-b], [b,a]]$
	where $a, b \in \mathbb{R}$ and $B$ is not the zero matrix. 
	 Let $\groupop$ be the matrix multiplication operator, then system~(\ref{eq:simplelinear}) is $\Gamma$-equivariant.
	
\end{example}

\begin{example}
Lorenz attractor models the two-dimensional motion of a fluid in a container. Its dynamics are as follows:
\begin{align}
\label{eq:lorenz}
\dot{x} = -px + py, \dot{y} = -xz + rx - y, \dot{z} = xy - bz. 
\end{align}
where $p,r,$ and $b$ are parameters and $x,y$ and $z \in \mathbb{R}$.
Let $\Gamma$ be the group that contains $\gamma: (x,y,z) \rightarrow (-x,-y,z)$ and the identity map. Then, system~(\ref{eq:lorenz}) is $\Gamma$-equivariant\footnote{\url{http://www.scholarpedia.org/article/Equivariant_dynamical_systems}}.
\end{example}

\begin{example}
	\label{eg:car_trans}
	%\sayan{This is the unicycle model I think. Dubins model has a turning radius/length.}
Third, a car model is equivariant to the group of all translations of its position. The car model is described with the following ODEs:
\begin{align}
\label{eq:dubin}
\dot{x} = v \cos \theta, \dot{y} = v \sin \theta, \dot{\phi} = u, \dot{v} = a, \dot{\theta} = \frac{v}{L} \tan(\phi). 
\end{align}
where $u$ and $a$ can be any control signals and $x, y, v, \theta, $and $ \phi \in \mathbb{R}$. We denote $r = (x,y,v,\phi,\theta) = (p,\bar{p})$, where $p = (x,y)$. Let $\Gamma$ be the set of translations of the form $\gamma: r = (p,\bar{p})\rightarrow r' = (p + c,\bar{p})$, for all $c \in \mathbb{R}^2$. 
%Let it also consists of the maps $(x,y,\theta)\rightarrow (-x,-y,\theta +\pi)$, $(x,y,\theta)\rightarrow (-y,x,\theta +\pi/2)$ and $(x,y,\theta)\rightarrow (x,y,\pi/2)$. 
Then, system~(\ref{eq:dubin}) is $\Gamma$-equivariant.
\end{example} 

\begin{example}
	\label{ex:perm_cars}
	Consider the system of two cars with states $r_1$ and $r_2$. Let $\Gamma$ be the set containing the operator $\gamma: (r_1,r_2) \rightarrow (r_2,r_1)$ and the identity operator. Moreover, assume that $u$ and $a$ are the same for both cars. Then, the system is $\Gamma$-equivariant. 
\end{example}
\begin{example}
	
	Let $\Gamma$ be the group generated by the set of transformations of the form $\gamma: (r_1,r_2) = ((p_1,\bar{p}_1), (p_2,\bar{p}_2)) \rightarrow (r_1',r_2') = ((p_1 + c_1,\bar{p}_1), (p_2 + c_2,\bar{p}_2))$, where $c_1$ and $c_2 \in \mathbb{R}^2$, along with the group described in example~\ref{ex:perm_cars}. Then, the system is $\Gamma$-equivariant. Hence, the system is equivariant to translations in the positions of both cars. 
\end{example}

%\sayan{End with a complex example with multiple cars with interesting road geometry. Show informally permutation, together with translation, and rotation. }

%\begin{definition}
%	The set $\Gamma \cdot \xi(t)= \{ \gamma \cdot \xi(t) | \gamma \in \Gamma \}$ is called the group orbit of $\xi(t)$; thus, if we find one solution to an equivariant ordinary differential equation, the whole group orbit of this solution will also exist as solutions.
%\end{definition}


%Definitions.

%Examples.

%Well-known results for moving solutions.
% Should we put the result here?

\begin{comment}
\subsection{Types of Symmetry}
\label{sec:types}
In this section, we discuss the different types of symmetry operators that we consider in this paper, particularly in the experiments.


\paragraph{Linear Transformations for Linear Systems:} Assume that system~(\ref{eq:goal_ode}) is a linear system, i.e. $f(x) = A x$ for some $A \in \mathbb{R}^{n \times n}$ and for all $x \in \mathbb{R}^n$. Let $\Gamma$ be the group of linear operators acting on $\mathbb{R}^n$ that are invertible and commute with $A$, i.e. operators of the form $\gamma(x) = B x$, for all $x \in \mathbb{R}^n$ and for some $B \in \mathbb{R}^{n\times n}$,  where $AB = BA$ and $B^{-1}$ exists. Then, system~(\ref{eq:goal_ode}) is $\Gamma$-equivariant.
The correctness of this claim follows from the condition in Definition~\ref{def:equivariance} on the commutativity of $f$ and $\gamma$.

\paragraph{Permutations:} The third type of symmetry we consider is permutation. In systems with multiple agents such as platoons of cars or coupled oscillators, the identity of each agent does not matter in the evolution of the system. Hence, the system is equivariant to the group of permutations of the variables of the different agents in the state of the system. 

\paragraph{Limited Translations:} Some systems are equivariant for specific group of translation operators (translation vectors). For example, systems with trigonometric-based nonlinearities may be equivariant to fixed translation vectors in the angles in the state because of trigonometric identities.  


\paragraph{Arbitrary Translations:} Assume that a subset $D \subseteq [n]$ does not appear on the right-hand side of the differential equation, i.e. $f(x) = f(x')$ for all $x, x' \in \mathbb{R}^n$ such that $x_i = x_i'$ for all $i \in [n] \textbackslash D$. Moreover, let $\Gamma$ be the group of all operators that change the values of the components with indices in $D$. Then, $f$ is $\Gamma$-equivariant. This type of symmetry is common in kinematic models where the absolute position of the agent does not affect the dynamics.



These groups of operators are simple and are a first step toward a wider use of symmetry in safety verification of hybrid systems.


%This is where we develop the different types of symmetries for linear and nonlinear systems. Could be a long list of examples, or definitions. 
\end{comment}


==> types_of_sym.tex <==
\subsection{Types of Symmetry}
\label{sec:types}
In this section, we discuss the different types of symmetry operators that we consider in this paper, particularly in the experiments.


\paragraph{Linear Transformations for Linear Systems:} Assume that system~(\ref{eq:goal_ode}) is a linear system, i.e. $f(x) = A x$ for some $A \in \mathbb{R}^{n \times n}$ and for all $x \in \mathbb{R}^n$. Let $\Gamma$ be the group of linear operators acting on $\mathbb{R}^n$ that are invertible and commute with $A$, i.e. operators of the form $\gamma(x) = B x$, for all $x \in \mathbb{R}^n$ and for some $B \in \mathbb{R}^{n\times n}$,  where $AB = BA$. Then, (\ref{eq:goal_ode}) is $\Gamma$-equivariant.
The correctness of this claim follows from the condition in Definition~\ref{def:equivariance} on the commutativity of $f$ and $\gamma$.


\paragraph{Arbitrary Translations:} Assume that a subset $S\subseteq [n]$ does not appear on the right-hand side of the differential equation, i.e. $f(x) = f(x')$ for all $x, x' \in \mathbb{R}^n$ such that $x_i = x_i'$ for all $i \in [n] \textbackslash S$. Moreover, let $\Gamma$ be the group of all operators that change the values of the components with indices in $S$. Then, $f$ is $\Gamma$-equivariant. This type of symmetry is common in kinematic models where the absolute position of the agent does not affect the dynamics.

\paragraph{Permutations:} The third type of symmetry we consider is permutation. In systems with multiple agents such as platoons of cars or coupled oscillators, the identity of each agent does not matter in the evolution of the system. Hence, the system is equivariant to the group of permutations of the variables of the different agents in the state of the system. 

\paragraph{Limited Translations:} Some systems are equivariant for specific group of translation operators (translation vectors). For example, systems with trigonometric-based nonlinearities may be equivariant to fixed translation vectors in the angles in the state because of trigonometric identities.  

These groups of operators are simple and are a first step toward a wider use of symmetry in safety verification of hybrid systems.


This is where we develop the different types of symmetries for linear and nonlinear systems. Could be a long list of examples, or definitions. 


==> verif_algo_multiple_gamma.tex <==
\subsection{The $\multiplesymtree$ procedure}
\label{sec:verification_Gamma}
\vspace{-0.1in}

Procedure $\multiplesymtree$ (Algorithm~\ref{code:symmetry_Gamma}) is a generalization of $\symtree$ using a group of symmetries. The $\multiplesymtree$ procedure still does BFS over $\cachTree$, keeps track of the parts of the input initial set $\initialset_n$ that are not proven safe  (line~\ref{ln:leftstatesupdate_m}); returns $\auto{Unsafe}$ with the same logic (line~\ref{ln:sym_unsafe_m}), and return $\auto{Compute}$ in case there are parts of $\initialset_n$ that are not proven safe nor have refinements in $\cachTree$ (line~\ref{ln:compute_m}). 

The key difference from $\symtree$ is that different transformations may be useful at different nodes. This leads to the possibility of multiple nodes in $\cachTree$, that are not ancestors or descendants of each other, covering the same parts of $\initialset_n$ under different transformations. Recall that in $\symtree$, only ancestors cover the parts of $\initialset_n$ that are covered by their descendants since $\gamma$ is invertible. Hence, it was sufficient to not add the children of a node to $\traversalstack$ to know that the part it covers, by transforming its initial set, from $\initialset_n$ is safe (line~\ref{ln:NoIntersect}). However, it is not sufficient in $\multiplesymtree$ since there may be another node that cover the same part of $\initialset_n$ which has a transformed reachtube that intersects $U$, hence refining what already has been proven to be safe. The solution is to remove explicitly from $\initialset_n$ what has been proven to be safe (line~\ref{ln:leftstatesupdate_m}). 
Moreover, it cannot return $\auto{Compute}$ when the transformed reachtube of a visited node intersects $U$ and its children initial sets do not contain the part it covers from $\initialset_n$ as in line~\ref{ln:compute} of $\symtree$. That is because other nodes may cover that part because of the availability of multiple symmetries. Hence, it cannot return $\auto{Compute}$ unless it traversed the whole tree and still parts of $\initialset_n$ could not be proven to be safe.
%\vspace{-.3in}
\vspace{-0.1in}
\begin{algorithm}
	\small
	\caption{$\multiplesymtree$}
	$\label{code:symmetry_Gamma}$
	\begin{algorithmic}[1]
		\State \textbf{input:} $\unsafe$, $\Gamma$, $\cachTree$, $\initialset_n$
		\State $\initialset_c := \cachTree.\rootnode.\initialset$
		%\State $\Gamma \gets getGamma(\initialset_c,\initialset_n)$
		%\State $\theta_u := \coverstack.\stacktop.\theta$ \Comment{new initial set with uncomputed reachtube}
		%\State $\delta_u := \coverstack.\stacktop.\delta$
		\If {$ \initialset_n \not\subseteq\cup_{\gamma \in \Gamma} \gamma (\initialset_c)$ $\label{al2:if_m}$}
		\State \textbf{return:} $\auto{SymmetryNotUseful}$ \label{ln:symNotUseful_m}
		\EndIf
		\State $\leftstates \gets \initialset_n$
		%\State $\tempstack := \{\langle \theta_u,\delta_u, \epsilon_u\rangle\}$
		\State $\traversalstack := \{\cachTree.\rootnode\}$
		\While {$\traversalstack \neq \emptyset$ and $\leftstates \neq \emptyset$}\label{ln:while_symtree_m}
		\State $\node \gets \traversalstack.dequeue()$ \label{ln:dequeue_m}
		\State $\initialset_c := \node.\initialset$; $\{(R_i,t_i)_{i=0}^k\} = \node.sim$
		%\State $\Gamma \gets getGamma(\initialset_c, \initialset_n)$
		\State $X = \{x  : \exists \gamma \in \Gamma, x \in \gamma (\initialset_c ) \text{ and } \gamma (\node.\overrt) \cap U = \emptyset \}$ \label{ln:computingX_m}
		\State $\leftstates \gets \leftstates \textbackslash X$ \label{ln:leftstatesupdate_m}
		\If{$\exists \gamma \in \Gamma, j\ |\ \gamma (R_j)\ \cap \ U \neq \emptyset \text{ and } \gamma (R_0) \in \leftstates$} \label{ln:if_unsafe_m}
		\State Return $\auto{Unsafe}$ \label{ln:sym_unsafe_m}
		%\Elsif{$|\node.\nodechildren| < 2^n$}
		%\State
		\EndIf
		\If{$len(\node.\nodechildren) > 0$}
		\State $\traversalstack.enqueue(\node.\nodechildren)$ \label{ln:addChildren_m}
		\EndIf
		\EndWhile
		\If {$\leftstates \neq \emptyset$} \label{ln:if_not_empty_m}
		\State \bf{return:} $\auto{Compute}$ \label{ln:compute_m}
		\EndIf
		\State \textbf{return:} $\auto{Safe}$ \label{ln:sym_safe_m}
		%\algstore{myalg}
	\end{algorithmic}
\end{algorithm}
\vspace{-0.2in}
We show that $\multiplesymtree$ has the same guarantees as $\symtree$ in the following two theorems with the proof being in Appendix~\ref{sec:app_symtree_proofs_m}.
\begin{restatable}[Completeness]{theorem}{secondcompleteness}
	\label{thm:termination_m}
	If there exists a set of nodes $S$ in $\cachTree$, where each $s\in S$ has a corresponding set of transformations $\Gamma_s \subseteq \Gamma$, such that
	\vspace{-0.1in} 
	\[\initialset_n \subseteq \cup_{s \in S, \gamma_s \in \Gamma_s} \gamma_s(s.\initialset) \text{ and } U \cap \cup_{s \in S, \gamma_s \in \Gamma_s} \gamma_s(s.\overrt) = \emptyset,\] 
	$\symtree$ will return ${\sf{Safe}}$. Also, if there exists a $\node$ $s$ in $\cachTree$ and a $\gamma \in \Gamma$, where $\gamma(s.sim)$ intersects $U$ and starts from $\initialset_n$, then $\multiplesymtree$ will return $\auto{SymmetryNotUseful}$, ${\sf{Unsafe}}$, or ${\sf{Compute}}$.
\end{restatable}
\vspace{-0.1in} 
\begin{restatable}[Soundness]{theorem}{secondsoundness}
	\label{thm:sym-reach-sound_m}
 $\multiplesymtree$ is sound: if it returns ${\sf{Safe}}$, then the reachtube $\Rtube(\initialset_n,T)$ does not intersect $U$ and if it returns ${\sf{Unsafe}}$, then there exists a trajectory starting from $\initialset_n$ that enters the unsafe set. 
\end{restatable}



The new challenge in $\multiplesymtree$ is in computing the union at line~\ref{al2:if_m}, computing $X$ in line~\ref{ln:computingX_m} and in the $\exists$ in line \ref{ln:if_unsafe_m}. These operations depend on $\Gamma$ if it is finite or infinite and how easy is to search over it. We revisit the arbitrary translation from Section~\ref{sec:symmetry:cps} to show that these operations are easy to compute in some cases.
\vspace{-0.1in}

\subsection{Revisiting arbitrary translations}
\label{sec:rev_arbitrary_trans}
Recall that the car model in example~\ref{eg:car_trans} in Section~\ref{sec:symmetry:cps} is equivariant to all translations in its position. In this section, we show how to apply $\multiplesymtree$ not just for it, but to arbitrary differential equations. Let $D$ be the set of components of the states that do not appear on the RHS of (\ref{eq:goal_ode}) and $\Gamma$ be the set of all translations of the components in $D$. To check the $\mathit{if}$ condition at line~\ref{al2:if_m}, we only have to check if $\initialset_c$ projected to the $[n] \textbackslash D$ contains $\initialset_n$ projected to the same components. Since if it is true, $\initialset_c$ can be translated arbitrarily in its components in $D$ so that the union contains $\initialset_n$.


%Moreover, if $\initialset_n$ and all $\initialset$s in $\cachTree$ are projected to $[n] \textbackslash D$, then running $\multiplesymtree$ will be equivalent to that of $\symtree$ with $\gamma$ being the identity map. That is because all maps in $\Gamma$ in this example change only the components that belong to $D$, and if these variables are removed by projection, all the maps become the identity map.  

Given two initial sets $K$ and $K'$ and the reachtube starting from $K'$, we compute $\beta \subseteq \mathbb{R}^n$ such that $K'\downarrow_D \oplus \beta = K \downarrow_D$. Then, if $K \subseteq K'$, by Corollary~\ref{cor:reachtube_transform}, we can use that $\beta$ to compute an overapproximation of $\Rtube(K,T)$ by computing $\Rtube(K',T) \oplus \beta$. Then, let $\beta$ be such that $\initialset_c\downarrow_D \oplus \beta = \leftstates\downarrow_D$, in line~\ref{ln:computingX_m}. 
%If $\node.rt \oplus \beta$ intersects $U$, we will need to refine.
 We set $X$ to be equal to $\initialset_c \oplus \beta$ if $\node.rt \oplus \beta \cap U = \emptyset$ and to $\emptyset$, otherwise.
 %
 To check the $\exists$ operator in line~\ref{ln:if_unsafe_m}, we can treat the simulation as $\node.rt$ and compute $\beta$ accordingly. Then, compute $\node.sim \oplus \beta$. The new condition would be then: if $R_j \oplus \beta \cap U$. Notice that we dropped $\gamma(R_0) \in \leftstates$ from the condition since we know that $R_0 \in \leftstates$ and $\beta$ is bloating it to the extent it is equal to $\leftstates$. 
 \vspace{-0.1in}
 
 \paragraph{Optimized $\multiplesymtree$ for arbitrary translations}
 
 The size of $K'\downarrow_D$ above does not matter, i.e. even if it is just a point, one can compute $\beta$ so that it covers $K\downarrow_D$. Hence, instead of computing $\Rtube(K,T)$, we compute only $\Rtube(K',T)$ and then compute $\beta$ from $K$ and $K'$ and then bloat it. This decreases the number of dimensions that the system need to refine by $|D|$. This is in contrast with what is done in $\multiplesymtree$ where the reachtubes are computed without changing the initial set structure. This improvement resulted in verifying models in 1s when they take an hour on DryVR as shown in Section~\ref{sec:experiments}. We call this algorithm $\transoptimized$ and refer to it as version 2 of $\multiplesymtree$ when applied to arbitrary translation invariance transformations. 
 
 %Moreover, if $\initialset_n$ and all $\initialset$s in $\cachTree$ are projected to $[n] \textbackslash D$, then running $\multiplesymtree$ will be equivalent to that of $\symtree$ with $\gamma$ being the identity map. That is because all maps in $\Gamma$ in this example change only the components that belong to $D$, and if these variables are removed by projection, all the maps become the identity map. 
%Notice that for after removing $X$ from $\leftstates$ in line~\ref{ln:leftstatesupdate_m}, none of the components of $\leftstates$ in $[n]\textbackslash D$ would be affected since $\Gamma$ only modify components in $D$. So, if the refinement is happening in one of the components in $[n] \textbackslash D$,  
%If the refinement was in one of the components in $D$, then the projection of the initial set to $[n]\textbackslash D$ would not change. Both the current node and the refined one would be able to cover $\initialset_n \downarrow_D$. Hence, it is correct to set $X$ to $\emptyset$ since the child (refined) node will have a tighter reachtube, after adding $\beta$, of that of its parent.

% There is no reason to set $X$ to a part of $\initialset_c \oplus \beta$ since any $\initialset$ of a $\node$ in $\cachTree$ would cover the $\initialset_n$ in the components in $D$.

% to check the safety of the system starting from an initial set $K$, we can compute the reachtube of the system starting from a new initial set $K'$ that has a projection to the components in $[n]\textbackslash D$ equal to that of $K$ and is a point when projected to the components in $D$. Then, we get $\beta$ such that $K' \oplus \beta = K$. We use this $\beta$ to compute $\Rtube(K,T)$ by computing $\Rtube(K',T) \oplus \beta$. Then, we can refine in the components in $[n]\textbackslash D$ to get tighter reachtubes since the tube is the tightest possible in the components in $D$. 
%We call this method the {\sf fast} one. 


%The projection $\initialset_c \downarrow_D$ of $\initialset_c$ to the components in $D$ is a hyperrectangle. The projection $\leftstates\downarrow_D$ of $\leftstates$ to the components in $D$ is compact. Hence, there exists a finite number of translations of $\initialset_c \downarrow_D$ that have a union that covers $\initialset_n \downarrow_D$. To compute $X$ at line~\ref{ln:computingX_m}, we check which of these translations when applied to $\node.rt$ do not intersect $U$. The union of the corresponding translated initial sets is $X$. This may leave some states that are safe from being part of $X$ because there might be multiple sets of translations that cover $\leftstates$. This will make $\multiplesymtree$ return $\auto{Compute}$ more. 
%However, if $\initialset_c\downarrow_D$ is a point we define $\gamma^*$ to be the map as well just translate $\initialset_c$ to be at the center of $\leftstates$ and 

%To check the $\mathit{if}$ condition at line~\ref{ln:if_unsafe_m}, we define the translation and bloating map $\gamma^*$ to be the one that takes $R_0$ to a set of states that when projected to $D$ is equal to $\leftstates\downarrow_D$ and leaves all other dimensions unaltered. Then, we apply $\gamma^*$ to $R_j$, for all $j \in [k]$. If any intersects $U$, then it is $\auto{Unsafe}$.

%Note that we do not have to compute the reachtube from the whole given initial set $K$. We can consider instead $K'$ which when projected on $[n]\textbackslash D$ is equal to the projection of $K$ on the same components while it is a single point when projected on the components in $D$. Then, we can rely on $\Gamma$ to cover $K$ in line~\ref{al2:if_m} and to compute $X$ in line~\ref{ln:computingX_m}. This will decrease the dimensions that need refinement by $|D|$.

\begin{comment}

Let $\gamma^*$ be a map that translates $\initialset_n$ to the center of $\leftstates$ and makes its projection to the components in $D$ equal to that of $\leftstates$ when projected on the same components. Then, $X$ is equal to $\gamma^*(\initialset_c)$ if $\gamma^*(\node.rt) \cap U = \emptyset$, and equal to $\emptyset$, otherwise.
 We let $X$ at line~\ref{ln:computingX_m} to be equal to $\gamma(\initialset_c)$


Before discussing how to compute $X$ at line~\ref{ln:computingX_m} and check the $\mathit{if}$ condition at line~\ref{ln:if_unsafe_m}, we consider a simpler problem.
%Consider two axes aligned hyperrectangles $K_1$ and $K_2 \subset \mathbb{R}^n$ representing two initial sets of states. 
Assume that the projection of $\initialset_c$ to the components in $D$ is a point.
%and that we already computed the reachtube of the system starting from it.  
Then, if we want to use the computed reachtube to get as much as we can from the reachtube starting from $K_2$, we grid the box in $K_2$ that correspond to these variables with diameters equal to the diameters of $K_1$. On the boundaries, the cells of the grid may overlap but no extra states should be covered because of the griding. After that, we compute the translation vector that takes the center of $K_1$ to the center of each cell in the grid.  Then, we use these vectors to translate the computed reachtube and union them to get a reachtube for $K_2$. However, there might be exponential number of grid cells and we will need to translate the reachtube exponential number of times. This will slow computation and computing reachtube in the usual way may be faster.

To solve this issue, we define the following map $\gamma_b : X \rightarrow X'$. 
$\gamma_b$ takes a bounding box $X \subset \mathbb{R}^n$ as input and returns a bounding box $X'$. First, it translates $X$ by the difference between the center of $K_2$ from the center of $K_1$. Then, it adds to the upper bound in $X$ of a dimension $d$ that is translation invariant the difference between the upper bound of $K_2$ with the upper bound of the translated $K_1$, if the difference is positive, and adds to the lower bound the difference between the corresponding lower bounds, if the difference is negative.

%we may translate $K_1$ to the center of $K_2$ and then bloat the lower and upper bound of each translation invariant dimension to contain that of $K_2$. This is equivalent to translating $K_1$ several times above.
The following theorem relates the result of translating the reachtube that starts from $K_1$ several times and unioning the result as described above with applying $\gamma_b$ to the reachtube starting from $K_1$.
\begin{theorem} Let $\Gamma_g$ be the set of translations that move $K_1$ to the centers of the grid in $K_2$ and $\gamma_b$ be the transformation that translate $K_1$ to the center of $K_2$ and then increase the upper bound of the translated $K_1$ of each translation invariant dimension to match that of $K_2$ and decrease the corresponding lower bound similarly. Then,
	\[
	\cup_{\gamma \in \Gamma_g}\Rtube(\gamma(K_1), T) = \Rtube(\gamma_b(K_1), T) = \gamma_b(\Rtube(K_1,T)).
	\]
	Moreover, $\Rtube(\gamma_b(K_1), T) \supseteq \Rtube(K_2, T)$.
\end{theorem} 
\begin{proof}
	Note first that $\gamma_b(K_1) = \cup_{\gamma \in \Gamma_g} \gamma(K_1) \supseteq K_2$. Moreover, we know that $\cup_{\gamma \in \Gamma_g}\Rtube(\gamma(K_1), T) = \Rtube(\cup_{\gamma \in \Gamma_g} \gamma(K_1), T)$. Hence, the first equality. Also, by Theorem~\ref{thm:reachtube_transform}, $\Rtube(\gamma(K_1), T) = \gamma(\Rtube(K_1, T))$, for all $\gamma \in \Gamma_g$. Hence, $\cup_{\gamma \in \Gamma_g}\Rtube(\gamma(K_1), T) = \cup_{\gamma \in \Gamma_g}\gamma (\Rtube(K_1, T)) = \gamma_b (\Rtube(K_1, T))$. Therefore, $\gamma_b (\Rtube(K_1, T)) = \Rtube(\gamma_b(K_1), T)$. Finally, since $\gamma_b(K_1) \supseteq K_2$, the last inequality follows.
\end{proof}

\end{comment}
\vspace{-.1in}





==> verif_algo_thms.tex <==
\begin{restatable}[Completeness]{theorem}{firstcompleteness}
	\label{thm:termination}
	If there exists a set of nodes $S$ in $\cachTree$ with \[\initialset_n \subseteq \cup_{s \in S} \gamma(s.\initialset) \text{ and } U \cap \cup_{s \in S} \gamma(s.\overrt) = \emptyset,\] $\symtree$ will return ${\sf{Safe}}$. Also, if there exists a $\node$ $s$ in $\cachTree$ where $\gamma(s.sim) \cap U \neq \emptyset$ and starts from $\initialset_n$, then $\symtree$ will return $\auto{SymmetryNotUseful}$, ${\sf{Unsafe}}$, or ${\sf{Compute}}$.
\end{restatable}

\begin{comment}
\begin{proof}
We will prove the ${\sf{Safe}}$ and ${\sf{Unsafe}}$ cases separately. But first, note that $\symtree$ traverses $\cachTree$ in a BFS manner and $\cachTree$ is of finite size. Hence, $\symtree$ terminates. 
\paragraph{${\sf{Safe}}$} %The condition in the theorem implies that $U \cap \gamma(\node.\overrt) = \emptyset$ for all $\node \in S$. Moreover, the while loop at line~\ref{ln:while_symtree} traverses $\cachTree$ in a BFS manner. Hence, if any of these nodes got visited, i.e. dequeued at line~\ref{ln:dequeue}, the condition at line~\ref{ln:if_safe} will be true. That means that $\symtree$ will not return ${\sf{Unsafe}}$ or ${\sf{Compute}}$ in that iteration and none of its children will be enqueued in $\traversalstack$. 

First, the $\initialset$ of the root contains all the $\initialset$s in the tree. Hence, if the union of the transformation of the $\initialset$s of the nodes in $S$ under $\gamma$ contains $\initialset_n$, then so does $\gamma(\rootnode.\initialset)$. Then, $\symtree$ will not return $\auto{SymmetryNotUseful}$.

Second, we prove that $\symtree$ will not return ${\sf{Unsafe}}$. Assume that the condition at line~\ref{ln:if_unsafe} was taken at a given iteration where some node $\node_p$ is the one being visited. Then, $\gamma(\node_p.sim)$ starts from $\initialset_n$ and intersects $U$. By Theorem~\ref{thm:reachtube_transform}, this is a simulation of the system that starts from $\gamma(\node_p.sim.R_0)$.  However, by the assumption of the current theorem, there exists a $\node_c \in S$ with $\node.\initialset_c$ that contains $\gamma(\node_p.sim.R_0)$. Moreover, from Definition~\ref{def:discrepancy} and $\simVerif$, we know that simulation belongs to $\node_c.\overrt$. But, $\node_c.\overrt \cap U = \emptyset$, contradiction. Hence, the condition at line~\ref{ln:cond_addChildren} could not be taken under the assumptions of the theorem.

%Moreover, if some $\node \in S$ was never visited in the while loop, that means that its parent or one of its grandparents in $\cachTree$ was visited in some iteration and the condition at line~\ref{ln:cond_addChildren} was not taken in that iteration. Let us name that parent or grandparent $\node_p$. 

Third, we will prove that $\symtree$ will not return ${\sf{Compute}}$. Assume for the sake of contradiction that it returned ${\sf{Compute}}$ at a given iteration and $\node_p$ was the node being visited. Then, all the conditions in the while loop were not satisfied. Hence, there exists subset $\gamma(\node_p.\initialset) \cap \initialset_n$ that is not covered by the transformed initial sets of the children of $\node_p$. Since $\gamma$ is inveritble and the initial sets of the children  are disjoint, then that part would not be covered by other nodes in the tree other than $\node_p$ and its parent and grandparents. However, all of these parent nodes have $\overrt$ that intersect $U$ for them to got refined in the first place. Hence, none of them belong to $S$. Therefore, there is no node in $S$ with $\initialset$ that cover that part. That contradicts our assumption that the union of $\initialset$s of nodes in $S$ contains $\initialset_n$. Therefore, $\symtree$ does not return ${\sf{Compute}}$ under the assumptions of the theorem.

Finally, since the algorithm terminates and it would not return ${\sf{Compute}}$, ${\sf{Unsafe}}$, or $\auto{SymmetryNotUseful}$, it will return ${\sf{Safe}}$.

\paragraph{${\sf{Unsafe}}$} Let $\node_p$ be a node in $\cachTree$ with $\gamma(\node.sim)$ that starts from $\initialset_n$ and intersects $U$. Then, in the BFS traversal of $\cachTree$, for none of its parent and grandparents, the condition at line~\ref{ln:if_safe} will be true since $\node.sim \subseteq \node.\overrt$. Hence, $\symtree$ will either return ${\sf{Compute}}$, ${\sf{Unsafe}}$, or $\auto{SymmetryNotUseful}$ before visiting $\node_p$ or it will visit it and line~\ref{ln:if_unsafe} will be true. In that case, $\symtree$ will return ${\sf{Unsafe}}$.
\end{proof}
\end{comment}

\begin{restatable}[Soundness]{theorem}{firstsoundness}
	\label{thm:sym-reach-sound}
	$\symtree$ is sound: if it returns ${\sf{Safe}}$, then the reachtube $\Rtube(\initialset_n,T)$ does not intersect $U$ 
	 and if it returns ${\sf{Unsafe}}$, then there exists a trajectory starting from $\initialset_n$ that enters the unsafe set. 
\end{restatable}

\begin{comment}
\begin{proof}
	We will again separate the proofs for the ${\sf{Safe}}$ and ${\sf{Unsafe}}$ cases.
	\paragraph{${\sf{Safe}}$} If $\symtree$ returns ${\sf{Safe}}$, it means that the condition in line~\ref{al2:if} is not true. Moreover, in every iteration of the while loop, either the condition in line~\ref{ln:if_safe} or the one in line~\ref{ln:cond_addChildren} is taken. When the one in line~\ref{ln:if_safe} is taken, it means either that the node is useless for computing the reachtube starting from $\initialset_n$ or the reachtube does not intersect $U$. If the condition at line~\ref{ln:cond_addChildren} was taken, it adds children with union of the transformed $\initialset$s cover the part of $\initialset_n$ that was covered by the parent $\initialset$. Hence, none of the states in $\initialset_n$ will not be checked the safety for. Thus, every state in $\initialset_n$ will belong to some $\node.\initialset$ for which line~\ref{ln:if_safe} will be true. Therefore, the system starting from $\initialset_n$ is safe.
	\paragraph{${\sf{Unsafe}}$} Assume that the node visited in the iteration at which $\symtree$ returned ${\sf{Unsafe}}$ be $\node_p$. Then, $\gamma(\node_p.\sim)$ starts from $\initialset_n$ and intersects $U$. Moreover, by Theorem~\ref{thm:sol_transform}, it is the simulation of the system starting from $\node_p.\sim.R_0$. Hence, it is a counter example and the system is unsafe.                                                                                                                                                           
\end{proof}
\end{comment}


In summary, $\symtree$ shows that a single symmetry $\gamma$ could decrease the number of fresh reachtube computations needed for verification. Next, we revisit  Example~\ref{eq:simplelinear} to illustrate the need for multiple symmetry maps.


\paragraph{Circular orbits and scaling symmetry}
The linear system in Example~\ref{eq:simplelinear} has circular orbits. Consider the initial set $K = [[21.5,21.5],[24.5,24.5]]$, 
%where the first list represent the lower bounds for $x_1$ and $x_2$ and the second one, their upper bounds respectively. 
the unsafe set $x_2 \geq 32$ after $t = 1.4s$, and the time bound $T=1.5s$. Any matrix $B$ that commutes with $A$, the RHS of the differential equation, is a symmetry transformation. However, once this matrix is fixed, we do not change it as per $\symtree$. Any diagonal matrix that commutes with $A$ has equal diagonal elements. Such a matrix would scale $x_1$ and $x_2$ by the same factor. Hence, applying $B$ to any axis aligned box would either scale the box up or down on the diagonal. That means applying $B$ to $K$ wouldn't contain the upper left or bottom right partitions, but only possibly the bottom left corner. With  $B = [[0.95,0], [0, 0.95]]$, only one out of 7 reachtubes is obtained via transformation (first row of Table~\ref{table:experimental_results}). 

That is because we are using a single transform which leaves $\symtree$ in most of the input cases useless. Figure~\ref{fig:circle_nosym} shows the reachtube (colored green to  yellow) computed using $\simVerif$, unsafe set (brown). Figure~\ref{fig:circle_sym} shows the reachtube computed using $\simVerif$ and $\symtree$. The part of the reachtube that was computed using symmetry is colored between blue and violet.
The other part is still between yellow and green. Only the upper left corner has been transformed instead if being computed. Next, we present $\multiplesymtree$, a generalization of $\symtree$ that uses a group of symmetries aiming for a bigger ratio of transformed to computed reachtubes.

\vspace{-0.3in}


